Data-Dependent Randomized Smoothing

Randomized smoothing is a recent technique that achieves state-of-art performance in training certifiably robust deep neural networks. While the smoothing family of distributions is often connected to the choice of the norm used for certification, the parameters of these distributions are always set as global hyper parameters independent from the input data on which a network is certified. In this work, we revisit Gaussian randomized smoothing and show that the variance of the Gaussian distribution can be optimized at each input so as to maximize the certification radius for the construction of the smooth classifier. Since the data dependent classifier does not directly enjoy sound certification with existing approaches, we propose a memory-enhanced data dependent smooth classifier that is certifiable by construction. This new approach is generic, parameter-free, and easy to implement. In fact, we show that our data dependent framework can be seamlessly incorporated into 3 randomized smoothing approaches, leading to consistent improved certified accuracy. When this framework is used in the training routine of these approaches followed by a data dependent certification, we achieve 9% and 6% improvement over the certified accuracy of the strongest baseline for a radius of 0.5 on CIFAR10 and ImageNet.

==> Data-Dependent Randomized Smoothing-camera-ready/Sections/UAI_rebuttal.tex <==
\newpage
\section{Rebuttal}
\subsection{bfhi Score:5 Confidence:4}


\paragraph{Our response.} We thank the reviewer for the detailed feedback. We address the raised concerns from the reviewer in the same order. We are glad that the reviewer found the idea novel and intriguing and that it has a potential high impact within a subfield of AI.

\textbf{A memory-based based classifier means that its performance will depend on the data it previously saw, and it also depends on the order data comes in.} In general, the reviewer is correct about their observation and we have openly discussed this in the paper as stated in the Limitations Section E of the Appendix. However, observe that memory based certification is order dependent only if two differently predicted samples have overlapping certified regions, i.e. when either the middle or right most cases on Figure 2 occur. That is to say, if overlapping certified regions of different predictions does not occur, the memory based approach is order invariant. A natural question that arises is: ``How likely is it to have two certified regions, note that they are often of $\ell_2$ order of 1.0, intersect for two differently predicted samples?" We observe that this is far unlikely to occur, unless the accuracy of the classifier is poor. During memory based certification, we observe that for all experiments conducted on the respective datasets, this scenario does not happen. This implies that all reported certified accuracies in the paper are in fact the same for any arbitrary order of testing samples of the respective datasets.


\textbf{It seems to me it will become harder and harder to certify when more points are in memory. If there are infinite number of data coming in, what is the asymptotic performance of the proposed method? Would certified accuracy drop to 0 asymptotically? And how does the order of data affect its asymptotic performance?} The observation of dense ``infinite" data for testing is partially true. While indeed the more samples tested the more likely for an intersection of certified regions to happen, however, it is not necessarily the case that the intersections of certified regions of differently predicted samples will increase. To that end, this does not mean that all new samples will later be necessarily certified with consecutively smaller regions, as observed on the respective datasets, since intersected regions of differently classified samples are rare. However, this naturally suggests an interesting direction. A stronger adversary is one with a full access to the history of all previously tested samples in memory. Such an attacker can then present few malicious samples for testing that will go in memory such that for future samples this can cause the data dependent classifier to intersect with higher chances with previously differently predicted samples causing certified accuracy to asymptotically drop for future samples. While this adversary could exist in principal, it is also not practically of full relevance. This is since in practice classifiers at deployment get updated in which new classifiers with fresh new memory are to be certified. In general, this is an interesting future research direction, but currently, a definition of such a class of adversaries falls beyond the scope of our paper.

% Moreover, even in classical certification, attaining a certain certified accuracy performance on a dataset reflects the performance of such adversary

\textbf{Following the methodology in this paper, conceptually, we can also discard all the remembered certifications in memory, and start fresh with a new classifier each time. Essentially this means we are using one fresh classifier for each example. Is it possible to do so and what is the implication?} If one resets the memory and provide certification for every sample independently along with a certified radius, the best one can deduce from such a classifier is that if $x+\delta$ is presented to the classifier, to attain a sound certification, the same $\sigma$ used for $x$ should also be used for $x+\delta$. If such a condition can not be practically deployed, we only end up with a theoretical classifier (since we do not have a procedure to implement such a classifier with a constant $\sigma$ locally) that is with a sound certification. Thus, the memory here is to allow for a practical implementation of this classifier with a sound practical certification. Thus if the memory is reset consecutively when testing every one of the new $n$ samples, we are at either (1) providing a sound certification of $n$ tested samples for a theoretical classifier or (2) providing $n$ sound certifications for $n$ different smooth classifiers (each with a different $\sigma$). This is where the use of memory bridges this gap into providing a single practical classifier with a sound certification.



% This is since the randomized smoothing certification suggests that given $x$ if for all samples $x+\delta$ in the certified region of $x$ denoted as $\mathcal{R}(x)$ is predicted with a constant $\sigma$ prediction does not change.


\textbf{Is it possible to achieve soundness without memory?} Currently, we do not have any particular obvious approach to drop the dependence on previous samples for certification. This could be a potential future direction that we currently do not yet know how to approach.





% Note that as mentioned in Section 3.5, we found that this is the case in all of our experimental results where no instances with differently predicted labels share any overlap in their certified regions making our memory-enhanced classifier order invariant. 


\subsection{S8Ji Score:7 Confidence:3}
We thank the reviewer for the valuable and detailed comments. We are glad that our work was well-received by the reviewer.

\textbf{Regarding the dependent of the memory algorithm on the order.} Indeed, the reviewer comment is on spot in their observation. The memory algorithm is order dependent. We have openly discussed this in the paper as stated in the Limitations Section E of the Appendix. However, this drawback had no impact in all of our experimental results. As discussed in our response to Rerviewer bfhi, memory based certification is order dependent only if two differently predicted samples have overlapping certified regions, i.e. when either the middle or right most cases in Figure 2 occur. That is to say, if overlapping certified regions of different predictions does not occur, the memory based approach is order invariant. We observe that this it is is far to have intersection of two different certified regions of differently predicted samples. In all our experiments, we observe that this scenario does not happen (middle and right most settings of Figure 2). This implies that all reported certified accuracies in the paper are in fact the same for any arbitrary order of testing samples of the respective datasets.

\textbf{Regarding the constrained covariance matrix.} We agree with reviewer S8Ji. Anisotropic covariance matrices could increase the certified volume. However and for a fair comparison with earlier approaches such as SmoothADV and MACER, we devoted our analysis in this work for isotropic covariance matrices leaving the anisotropic counterparts for a future work. Moreover, considering full covariance matrices requires (1) deriving the resultant certificate (e.g. ellipsoid as opposed to $\ell_2$ balls) (2) defining a new approach towards comparing two anisotropic certified regions through volumes or other metrics.

\textbf{Regarding learning or predicting the variance.} This is an excellent idea that would alleviate the optimization cost of obtaining the optimal smoothing parameters. However, we argue that learning/predicting the smoothing parameters is a very challenging problem that could potentially reduce the improvement of using data dependent smoothing. We have had initial experiments of learning a separate network to predict $\sigma$ for the sole purpose of speeding up certification as this involves a forward pass through a network as opposed to solving the optimization problem. However, we do not find any particular gains, in fact this approach down performs the classical baselines as Cohen et al. We leave the investigation for this line of work for a future direction.


\subsection{MTkP Score:7 Confidence:3}
We thank the reviewer for the valuable and detailed comments. We are glad that our work was well-received by the reviewer.

\textbf{Regarding the runtime comparison}: We thank the reviewer for pointing out this fair comparison. We have included a detailed comparison of the running time in Appendix H. We will include this paragraph in the main paper in the final version.


\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{UAI22/rebuttal_figures/cohen_comparison_0.25.pdf}
    \caption{Rebuttal Experiment}
    \label{fig:rebuttal_experiment}
\end{figure}


\textbf{Regarding the minor issues.} We thank the reviewer for this insightful experiments. As suggested, we conducted this experiment for Cohen baseline at $\sigma=0.25$. We plot the histogram of the obtained $\sigma_x^*$ for CIFAR10 in orange. We also plot a histogram of the $\sigma_x^*$ at which the certified radius is improved in green. We report the results in Figure~\ref{fig:rebuttal_experiment}.
We found that the certified robustness improvements happen at the full spectrum of $\sigma_x^*$ showing the efficacy of our proposed data-dependent smoothing. We will include a more detailed version of this experiment in the final version.



\textbf{Regarding the proposed adjustment for the middle scenario in Fig 2.} The reviewer is correct about their observation and suggestion. We opted to the solution with the least computational overhead which is adjusting the radius of the new data as opposed to adjusting the radius of every intersected sample in memory. We would like to bring to the attention of the reviewer that in practice, given that the certified regions around every point is generally small, scenarios 2 and 3 in Figure 2 never happened on the correspondingly tested datasets, i.e. there are no differently predicted samples with intersected certified regions.

% However, better alternatives could exist that could potentially result in a better overall certified radius.
% There might exist many solutions for this case such as the one pointed out by the reviewer.


\textbf{Regarding $\hat x$ and $x'$}. Yes, this is indeed a typo where the optimization is over the adversary $x'$. We will correct this in a potential future version.

% We refer to $\hat x$ as the adversarial attack. $x'$ is the optimization variable in the objective:
% \[\max_{x'} -\log \mathbb {E}_{\epsilon \sim \mathcal N (0,\sigma^2I)} \left[f^y_{\theta}(x' + \epsilon)\right], \qquad \text{where}\quad \|x'-x\| \leq \zeta
% \]
% We will make this clearer in the final version.







\subsection{7p67 Score:7 Confidence:2}
We thank the reviewer for the valuable and detailed comments. We are glad that our work was very well-received with generally positive feedback by the reviewer.

\textbf{Regarding the presentation details.} We thank the reviewer for spotting some typos and fir suggesting several few ways to improve presentation. We will surely address those in any potential camera ready version.

% We have used the command eqref to refer to previous equations so that the reader could click on it to jump directly to the equation. We will fix this as per the suggestion and add paranthesis for better clarification.

% (2) We thank the reviewer for spotting this clerical error which will be fixed in the final version.

\textbf{Regarding predicting $\sigma^*$ for any $x$.} We thank the reviewer for sharing this interesting idea. We thought about learning $\sigma_x^*$ through a network that is jointly trained with the classifier. However, and due to the hardness of the problem, we were not able to attain robustness improvements from that approach over the Cohen et al baseline. The loss function used is similar to Equation 2, but the optimization is over parameters $\phi$ of an encoder network where $\epsilon$ is sampled from the encoder network. This is in similar spirit to variational autoencoders (VAEs). The reason for why this approach did not work could be attributed to several factors such as the poor performance of the classifier at early epochs, the complexity of the optimization, etc. Nevertheless, we believe that such approaches, if succeeded, would have several advantages such as alleviating the optimization cost.

==> Data-Dependent Randomized Smoothing-camera-ready/Sections/abstract.tex <==
\begin{abstract}
    Randomized smoothing is a recent technique that achieves state-of-art performance in training certifiably robust deep neural networks. While the smoothing family of distributions is often connected to the choice of the norm used for certification, the parameters of these distributions are always set as global hyper parameters independent from the input data on which a network is certified. In this work, we revisit Gaussian randomized smoothing and show that the variance of the Gaussian distribution can be optimized at \emph{each} input so as to maximize the certification radius for the construction of the smooth classifier. \textcolor{black}{Since the data dependent classifier does not directly enjoy sound certification with existing approaches, we propose a memory-enhanced data dependent smooth classifier that is certifiable by construction.} This new approach is generic, parameter-free, and easy to implement. In fact, we show that our data dependent framework can be seamlessly incorporated into 3 randomized smoothing approaches, leading to consistent improved certified accuracy. When this framework is used in the training routine of these approaches followed by a data dependent certification, we achieve 9\% and 6\% improvement over the certified accuracy of the strongest baseline for a radius of 0.5 on CIFAR10 and ImageNet.
\end{abstract}


% Our implementation can be found at
% \href{https://github.com/MotasemAlfarra/Data_Dependent_Randomized_Smoothing}{https://github.com/MotasemAlfarra/Data-Dependent-Randomized-Smoothing}

% \BG{shouldnt this be training and testing?}

% \cite{salman2020black}
% \bibi{Thing to stay consistent with throughout the paper. \\
% (1) do not use "data-dependent" instead use "data dependent"} \\
% \bibi{Use Cifar-10 or CIFAR10} \\
% \bibi{Change GA to Cohen et al}
% \bibi{We will not use any hyphenation  and no spaces (e.g. huyperparameters)}
% \bibi{We will always use \eg and \ie}

% \bibi{use MCMC maybe not Monte Carlo}
% \bibi{use MCMC maybe not Monte Carlo}

==> Data-Dependent Randomized Smoothing-camera-ready/Sections/conclusion.tex <==
% \vspace{-6pt}
\section{Conclusion}
% \vspace{-6pt}
In this work, we presented a simple and generic framework to equip randomized smoothing techniques with data dependency.
% Moreover, we provide a simple approach based on memory to certifying the data dependent classifier. We would like to emphasize that this approach is orthogonal to any smoothing training framework.
We demonstrated that  combining data dependent smoothing with 3 randomized smoothing techniques provided substantial improvement in their certified accuracy. 

==> Data-Dependent Randomized Smoothing-camera-ready/Sections/experiments.tex <==
\section{Experiments}



We conduct two sets of experiments to validate our key contributions. (\textbf{i}) We show that we can boost certified accuracy for several pre-trained models by using Algorithm \ref{alg:RS_DS} for data dependent smoothing only during certification, \ie without employing any additional training. (\textbf{ii}) Once data dependent smoothing is employed during training, we can improve the certified accuracy even further.
% (Algorithms \ref{alg:RS_DS} and \ref{alg:DS_DS}).
Since our framework is agnostic to the training routine, we incorporate it
% to the best of our knowledge, 
into 
% the only three methods that employ randomized smoothing as part of training, namely 
(\textbf{i}) \textsc{Cohen} \citep{cohen2019certified}, (\textbf{ii}) \textsc{SmoothAdv} \citep{salman2019provably} and (\textbf{iii}) \textsc{MACER} \citep{zhai2020macer}. Throughout, we use $\text{DS}$ to refer to when data dependent smoothing is  used only in certification and $\text{DS}^2$ when it is used during both training and certification.

% \BG{consider using \textsc{\textsc{Cohen}}, \textsc{\textsc{SmoothAdv}}, and \textsc{\textsc{MACER}} instead; they look nicer this way}



\textbf{Setup.} 
We conduct experiments with ResNet-18 and ReNet-50 \citep{resnet} on CIFAR10 \citep{cifars} and ImageNet \citep{imagenet}, respectively. For CIFAR10 experiments, we train from scratch for 200 epochs. For ImageNet, we initialize using the network parameters provided by the authors. When $\sigma$ is fixed and following prior art, \eg \textsc{Cohen}, \textsc{SmoothAdv}, and \textsc{MACER}, we set $\sigma \in \{0.12, 0.25, 0.50\}$ and $\sigma \in \{0.25, 0.50, 1.0\}$ for CIFAR10 and ImageNet, respectively, for training and certification. We set $\alpha=10^{-4}$ in Algorithm \ref{alg:RS_DS} and the initial $\sigma_0$ to the $\sigma$ used in training the respective model. Unless stated otherwise, we set $n=1$ in Algorithm \ref{alg:RS_DS}. Following \textsc{Cohen} and \textsc{SmoothAdv}, we compare models using the approximate certified accuracy curve (simply referred to as certified accuracy) followed by the envelope curve over all $\sigma$. We also report the Average Certified Radius (ACR) proposed by MACER $\nicefrac{1}{|\mathcal S_{test}|} \sum_{(x,y)\in\mathcal S_{test}}  R(f_\theta, x).\mathbbm{1}\{\argmax_c g^c_\theta(x) = y\}$, where $\mathbbm{1}\{.\}$ is an indicator function. Following \textsc{Cohen}
% \footnote{We use the available code of \cite{cohen2019certified} to report all certification results in the paper for a given $\sigma$.}
and all randomized smoothing methods, we certify all results using $N_0=100$ Monte Carlo samples for prediction and $N=100,000$ estimation samples to estimate the radius with a failure probability of $0.001$ given a smoothing $\sigma$.
\input{ figs/Cohen}
\input{ tables/Cohen}

% where $\mathbbm{1}$ is an indicator function and $R$ is the radius in Equation \eqref{eq:certification_radius}.


\input{ figs/SmoothAdv}
\input{ tables/SmoothAdv}

\subsection{\textsc{Cohen} + DS}
% \vspace{-0.15cm}

We combine data dependent smoothing with \textsc{Cohen}. Following Gaussian augmentation, this method trains $f_\theta$ on $(x+\epsilon)$, where $\epsilon \sim \mathcal N (0,\sigma^2I)$, with the cross entropy loss.

% \vspace{-0.10cm}
\textbf{DS for certification only.} We first certify the trained models with the same fixed $\sigma$ used in training for all inputs, dubbed \textsc{Cohen}. Then, we certify using the memory based certification the same trained models with the proposed data dependent $\sigma_x^*$ produced by Algorithm \ref{alg:RS_DS}, which we refer to as $\text{\textsc{Cohen}-DS}$. Figure \ref{fig:GA} plots the certified accuracy for CIFAR10 and ImageNet in the first and second rows, respectively. Even though the base classifier $f_\theta$ is identical for $\text{\textsc{Cohen}}$ and $\text{\textsc{Cohen}-DS}$, Figure \ref{fig:GA} shows that $\text{\textsc{Cohen}-DS}$ is superior to $\text{\textsc{Cohen}}$ in certified accuracy across almost all radii and for all training $\sigma$ on both datasets. This is also evident from the envelope plots in the last column of Figure \ref{fig:GA}.
% reporting the best certified accuracy per radius over all $\sigma$ trained models.
In Table \ref{tb:Cohen}, we report the best certified accuracy per radius over all training $\sigma$ for $\text{\textsc{Cohen}}$ (envelope figure) against our best $\text{\textsc{Cohen}-DS}$, cross-validated over all training $\sigma$ and the number of iterations in Algorithm \ref{alg:RS_DS} $K$, accompanied with the corresponding ACR score. For instance, we observe that data dependent certification $\text{\textsc{Cohen}-DS}$ can significantly boost certified accuracy at radii $0.5$ and $0.75$ by $7.7\%$ (from $40.1$ to $47.8$) and $9.1\%$ (from $29.2\%$ to $38.3\%$), respectively, and by $0.193$ ACR points on CIFAR10. Moreover, we boost the certified accuracy on ImageNet by $4.6\%$  and $3.2\%$ at $0.5$ and $0.75$ radii, respectively, and by $0.159$ ACR points. 


% \vspace{-0.10cm}
\textbf{DS for training and certification.} We employ data dependent smoothing in both training and certification for \textsc{Cohen} models (denoted as $\text{\textsc{Cohen}-DS}^2$) by running Algorithm \ref{alg:DS_DS}. For CIFAR10, we train $\text{\textsc{Cohen}}$ first with fixed $\sigma$ for 50 epochs, \ie $K=0$ in Algorithm \ref{alg:RS_DS}, and then we perform data dependent smoothing with $K=1$ for the remaining 150 epochs. For ImageNet experiments, we only finetune the provided models for 30 epochs using Algorithm \ref{alg:DS_DS} with $K=1$. Once training is complete, we certify all trained models with Algorithm \ref{alg:RS_DS} using the memory based certification. In Figure \ref{fig:GA}, we observe that $\text{\textsc{Cohen}-DS}^2$ can further improve certified accuracy across all trained models on both CIFAR10 and ImageNet. This is also evident in the last column of Figure \ref{fig:GA} that shows the best certified accuracy per radius (envelope) over all training $\sigma$. We note that $\text{\textsc{Cohen}-DS}^2$ improves the certification accuracy of $\text{\textsc{Cohen}-DS}$ by $2.6\%$ and by $0.9\%$ at radii $0.5$ and $0.75$ respectively on CIFAR10, and by $4.8\%$ and $1.8\%$ at radii $0.5$ and $0.75$ respectively on ImageNet. The improvements are consistently present over a wide range of radii on both datasets. We do observe that the ACR score for $\text{\textsc{Cohen}-DS}^2$ on CIFAR10 marginally drops compared to $\text{\textsc{Cohen}-DS}$. We believe that this is due to the fact that some inputs that are classified correctly at the small radii have an overall larger certification radius for $\text{\textsc{Cohen}-DS}$ compared to $\text{\textsc{Cohen}-DS}^2$ on CIFAR10. Regardless, $\text{\textsc{Cohen}-DS}^2$ substantially 
outperforms $\text{\textsc{Cohen}}$ by $0.173$ ACR points. As compared to $\text{\textsc{Cohen}-DS}$, $\text{\textsc{Cohen}-DS}^2$ improves the ACR on ImageNet  from $1.257$ to $1.319$.


% \vspace{-0.15cm}
\subsection{\textsc{SmoothAdv} + DS}
% \vspace{-0.15cm}
We combine our data dependent smoothing strategy with the more effective \textsc{SmoothAdv}, which trains the smoothed classifier for every $x$ on the adversarial example $\hat{x}$ that maximizes $-\log \mathbb {E}_{\epsilon \sim \mathcal N (0,\sigma^2I)} \left[f^y_{\theta}(x' + \epsilon)\right]$, where $\|x'-x\| \leq \zeta$.%\BG{consider changing the variable from $\delta$ to something else; you used $\delta$ as the vector perturbation in Section 3.2}
% \begin{align*}
% \hat{x} = \argmax_{\|x'-x\| \leq \delta} ~-\log \mathbb {E}_{\epsilon \sim \mathcal N (0,\sigma^2I)} \left[f_{\theta}(x' + \epsilon)\right].
% \end{align*}
For CIFAR10 experiments, we follow  the training procedure of \textsc{SmoothAdv}, where the adversary $\hat{x}$ is computed with 2 PGD (proximal gradient descent) steps with $\zeta = 0.25$ and one augmented sample to estimate the expectation. For ImageNet experiments, we use the best reported models, in terms of certified accuracy, provided by the authors, which correspond to $\zeta = 0.5$ for $\sigma = 0.25$ and $\zeta = 1.0$ for $\sigma \in \{0.5, 1.0\}$.

\input{ figs/MACER}
\input{ tables/MACER}
% \vspace{-0.10cm}
\textbf{DS for certification only.} Similar to \textsc{Cohen}, we first certify \textsc{SmoothAdv} models trained with the same fixed $\sigma$. Then, we certify the proposed data dependent $\sigma_{x}^*$ models using the memory-based certification, which we refer to as $\text{\textsc{SmoothAdv}-DS}$. In Figure \ref{fig:SmoothAdv}, we show the certified accuracy for both CIFAR10 and ImageNet in the first and second rows, respectively. The last column shows the envelopes per radius. Even though they both share the same classifier $f_\theta$, $\text{\textsc{SmoothAdv}-DS}$ significantly improves upon $\text{\textsc{SmoothAdv}}$ over all radii and all values of $\sigma$ in training for both CIFAR10 and ImageNet. In particular, for models trained with $\sigma=0.25$, $\text{\textsc{SmoothAdv}}$ achieves a zero certified accuracy for large certification radii ($\ge 1.0$), while $\text{\textsc{SmoothAdv}-DS}$ achieves non-trivial certified accuracy in these cases. Similar to the earlier setup, we report the best certified accuracy along with the ACR scores in Table \ref{tb:SmoothAdv}. We improve over $\text{\textsc{SmoothAdv}}$ by large margins. For example, the certified accuracy at $0.5$ radius increases by $5.4\%$ and $2.8\%$ on CIFAR10 and Imagenet, respectively. The improvement is consistent over all radii. The ACR also improves by $0.118$ and $0.158$ on CIFAR10 and ImageNet, respectively.



% \vspace{-0.10cm}
\textbf{DS for training and certification.} 
We fine tune the $\text{\textsc{SmoothAdv}}$ trained models (either the retrained CIFAR10 models or the ImageNet models provided by \textsc{SmoothAdv}) using Algorithm \ref{alg:DS_DS}, where $\sigma_x^*$ is computed using Algorithm \ref{alg:RS_DS}. We report the per $\sigma$ certification accuracy comparing $\text{\textsc{SmoothAdv}-DS}^2$ (certified also using memory based certification) to both $\text{\textsc{SmoothAdv}-DS}$ and $\text{\textsc{SmoothAdv}}$. $\text{\textsc{SmoothAdv}-DS}^2$ further improves the certified accuracy as compared to $\text{\textsc{SmoothAdv}-DS}$ with performance gains more prominent on ImageNet. While the improvement of $\text{\textsc{SmoothAdv}-DS}^2$ over $\text{\textsc{SmoothAdv}-DS}$ is indeed small, \eg $0.7\%$ at radius $0.5$ on CIFAR10, we observe that the performance gaps are much larger on ImageNet reaching  $1.4\%$ at $0.5$ radius as shown in Table \ref{tb:SmoothAdv}. We see a similar trend in ACR with improvements of $0.013$ and $0.069$ on CIFAR10 and ImageNet, respectively. $\text{\textsc{SmoothAdv}-DS}^2$ boosts the certified accuracy of $\text{\textsc{SmoothAdv}}$  at radius 0.5 by $6.1\%$ and $4.2\%$ on CIFAR10 and ImageNet, respectively.




\input{ figs/qualitative}

% \vspace{-0.15cm}
\subsection{\textsc{MACER} + DS}
% \vspace{-0.15cm}
We integrate data dependent smoothing within \textsc{MACER} which trains $g_\theta$ by minimizing over the parameters $\theta$ the following objective
% updates model parameters using a regularization that encourages a maximum certification radius, as follows:
% \vspace{-2pt}
$
% \begin{align*}
% \min_\theta 
-\log g_\theta(x) + \frac{\lambda \sigma}{2} \max\left (\gamma - \frac{2R}{\sigma} , 0\right).\mathbbm{1}\{\argmax_c ~g^c_\theta(x) = y\}.
% \end{align*}
$ where $R$ also depends on $\theta$. While this seems to be similar in spirit to our approach, we in fact maximize the certification radius over $\sigma$ with fixed parameters $\theta$ for every $x$. 
% The expectations in the loss are approximated with Monte Carlo sampling.
We conduct experiments on CIFAR10
% \footnote{ResNet-50 trained models on ImageNet are not provided by the authors.
% Training them from scratch is prohibitively expensive.
% } 
following the training procedure of \textsc{MACER} estimating the expectation with $64$ samples, $\lambda = 12$, and $\gamma = 8$. We set $n=8$ in Algorithm \ref{alg:RS_DS} with ablations on $n=1$ in the \textbf{appendix}.


% \vspace{-0.10cm}
\textbf{DS for certification only.} Similar to the earlier setup in \textsc{Cohen} and \textsc{SmoothAdv}, we certify models with fixed $\sigma$ and then with data dependent $\sigma^*_x$ using the memory based certification, referred to as $\text{\textsc{MACER}-DS}$. In Figure \ref{fig:MACER}, we observe that $\text{\textsc{MACER}-DS}$ significantly outperforms $\text{\textsc{MACER}}$ particularly in the large radius region. This can also be seen in the envelope figure reporting the best certified accuracy per radius over $\sigma$. Similarly, Table \ref{tb:MACER} demonstrates the benefits of data dependent smoothing, where it boosts certified accuracy by $7.4\%$ (from $59.3\%$ to $66.7\%$) and $8.7\%$ ($43.6$ to $52.3$) at $0.25$ and $0.5$ radii, respectively. Moreover, we improve ACR by $0.139$ points.

% \vspace{-0.10cm}
\textbf{DS for training and certification.} We incorporate data dependent smoothing as part of \textsc{MACER} training and certification in a similar fashion to the earlier setup, dubbed $\text{\textsc{MACER}-DS}^2$. Figure \ref{fig:MACER} shows the improvement of $\text{\textsc{MACER}-DS}^2$  over the certification only $\text{\textsc{MACER}-DS}$ over all trained models. Table \ref{tb:MACER} summarizes the best certified accuracy per radius. Overall, we find that the performance is comparable or slightly better than $\text{\textsc{MACER}-DS}$, which is still significantly better than $\text{\textsc{MACER}}$ by $8.67\%$ at radius $0.5$. We also observe that  $\text{\textsc{MACER}-DS}$ enjoys better ACR than $\text{\textsc{MACER}-DS}^2$ with both being far better than the  $\text{\textsc{MACER}}$ baseline.
% \input{ figs/iteration_ablation}
% \input{ figs/appendix_visualization_\textsc{Cohen}}
% \input{ figs/appendix_visualization_\textsc{SmoothAdv}}


\begin{figure}
% \vspace{-0.95cm}
    \centering
        \includegraphics[width=0.23\textwidth]{ figures/iterations/CIFAR10_Adv_smooth_DS_DS_sigma_012.png}
        \includegraphics[width=0.23\textwidth]{ figures/iterations/ImageNet_Adv_smooth_RS_DS_sigma_050.png}
    \caption{\textbf{Varying %the number of iterations
    $K$ in Algorithm \ref{alg:DS_DS}.} Left figure shows certification with $\sigma_0=0.12$ on CIFAR10 and $\sigma_0=0.5$ on ImageNet is shown at the right.}
    \label{fig:iteration} 
\end{figure}

\subsection{DS for $\ell_1$ Certificates}

\textcolor{black}{At last, we extend our methodology to $\ell_1$ certification. We leveraged the results of \cite{yang2020randomized} that derived the tightest $\ell_1$ certificate using randomized smoothing with uniform distribution $\mathcal U[-\lambda, \lambda]^d$. The certified radius in that case has the form $\mathcal R_1 = \lambda(p_A - p_B)$. We replace our objective in Equation \eqref{eq:our_objective_v2} with:
\begin{equation}
\label{eq:our_objective_2}
\begin{aligned}
\lambda_x^* = &\text{arg}\max_\lambda \lambda \Bigg(\mathbb E_{\epsilon\sim \mathcal{U}[-\lambda, \lambda]^d}(f_\theta^{c_A}(x+\epsilon)) \\
&- \max_{c \neq c_A} \mathbb E_{\epsilon\sim \mathcal{U}[-\lambda, \lambda]^d}(f_\theta^{c}(x+\epsilon))  \Bigg).
\end{aligned}
\end{equation}
% \begin{equation}
% \begin{align*}
% \end{align*}
% \end{equation}
% \begin{equation}
% \label{eq:our_objective}
% \begin{aligned}
%     \sigma^*_x =&\argmax_{\sigma} ~\frac{\sigma}{2} \Bigg(\Phi^{-1}\left( \mathbb{E}_{\epsilon \sim \mathcal{N}(0,\sigma^2I)}[f_\theta^{c_A}(x+\epsilon)]\right)  \\ \,\, - \,\, & \Phi^{-1}\left(\max_{c \neq c_A} \mathbb{E}_{\epsilon \sim \mathcal{N}(0,\sigma^2I)}[f_\theta^c(x+\epsilon)]\right) \Bigg).
% \end{aligned}
% \end{equation}
We solved our objective in Eq~\eqref{eq:our_objective_v2} in an identical fashion to our Algorithm \ref{alg:RS_DS} with the same hyperparameters for $\lambda \in \{0.25, 0.5, 1.0 \}$ in certification on both CIFAR10 and ImageNet. Further, we combine our data-dependent smooth classifier with the memory based algorithm proposed in Section~\ref{sec:memory-algorithm}. It is worthwhile mentioning that similar to the $\ell_2$ case, the memory based algorithm did not find any overlap between the certified regions of any pair of instances.
We report the results in Table \ref{tab:l1}. We observe that, similar to our extensive experiments on the $\ell_2$ certificate, our proposed memory-enhanced data-dependent smoothing yields consistent improvement in the $\ell_1$ certified accuracy. We report an improvement  of 7\% and 3\% over the state of the art certified accuracy at $\ell_1$ radius of 0.5 on CIFAR10 and ImageNet, respectively. At last, we note similar improvement to the $\ell_1$ ACR as reported in Table \ref{tab:l1}.
}


% \vspace{-0.15cm}
\subsection{Discussion and Ablation}
% \vspace{-0.15cm}
\textbf{Varying $K$.} We pose the question: does attaining better solutions to our proposed Objective \ref{eq:our_objective_v2} improve certified accuracy? To answer this, we control the solution quality of $\sigma_x^*$ by certifying trained models with a varying number of stochastic gradient ascent iterations $K$ in Algorithm \ref{alg:RS_DS}. In particular, we certify the trained models $\text{\textsc{SmoothAdv}-DS}^2$ and $\text{\textsc{SmoothAdv}-DS}$ on CIFAR10 and ImageNet, respectively, with a varying $K$. We leave the rest of the experiments for other models to the \textbf{appendix}. We observe in Figure \ref{fig:iteration} that the certified accuracy per radius consistently improves as $K$ increases, particularly in the large radius regime. This is expected, since Algorithm \ref{alg:RS_DS} produces better optimal smoothing $\sigma_x^*$ per input $x$ with larger $K$, which in turn improves the certification radius leaving room for improvements with more powerful optimizers.
% \footnote{Greedy heuristics solving Equation \ref{eq:our_objective_v2} are in the \textbf{appendix}, as they perform far worse than our approach.}. 



% \vspace{-0.10cm}
\textbf{Visualizing $\sigma^*_x$.} We show the variation of $\sigma^*_x$ that maximizes the certification radius over different inputs $x$. Figure  \ref{fig:qualitative} shows two examples, where the first and fourth columns contain the clean images. In the second column, a choice of fixed $\sigma=0.5$ is too large compared to our estimated  $\sigma^*_x=0.368$ that maximizes the certification radius as per Algorithm \ref{alg:RS_DS}. As for the fifth column, we observe that a constant $\sigma=0.25$ is far less than $\sigma^*_x=0.423$. This indicates that indeed the $\sigma^*_x$ maximizing the certification radius varies significantly over inputs. 

% \vspace{-0.10cm}
% \textbf{Runtime.} We measure the certification runtime on an NVIDIA Quadro RTX-6000 GPU for our proposed data dependent smoothed classifier (time includes Algorithm \ref{alg:RS_DS} in addition to the memory based certification) compared to the certification of a fixed $\sigma$ classifier. Certifying one CIFAR10 test input with ResNet18 takes 1.6 and an average of 1.8 seconds for a fixed $\sigma$ classifier and for the data dependent classifier ($K = 900$), respectively. Certifying an ImageNet test input on ResNet50 takes 109.5 and an average of 136 seconds for a fixed $\sigma$ classifier and our data dependent classifier ($K=400$), respectively. The runtime overhead added by
% using Algorithm \ref{alg:RS_DS} and memory based certification is negligible compared to the gains in certified accuracy.






% \begin{figure*}[t]
%      \centering
%      \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{ICLR22/new_figures/l1_cifar10-0.25.png}
%      \end{subfigure}
%     %  \hfill
%      \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{ICLR22/new_figures/l1_cifar10-0.5.png}
%      \end{subfigure}
%     %  \hfill
%      \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{ICLR22/new_figures/l1_cifar10-1.0.png}
%      \end{subfigure}
%     % \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{ICLR22/new_figures/l1_imagenet-0.25.png}
%      \end{subfigure}
%     %  \hfill
%      \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{ICLR22/new_figures/l1_imagenet-0.5.png}
%      \end{subfigure}
%     %  \hfill
%      \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{ICLR22/new_figures/l1_imagenet-1.0.png}
%      \end{subfigure}
%         \caption{
%         \textcolor{black}{ 
%         \textbf{$\ell_1$ Certified accuracy comparison against $\text{Yang}$ per radius per $\sigma$.} We compare $\text{Yang}$ against
%         % our data dependent certification
%         $\text{Yang-DS}$.
%         % and when data dependency is incorporated in both training and certification
%         % for several $\sigma$. 
%       We show CIFAR10 and ImageNet results in first and second rows, respectively. Similar to the earlier experiments on $\ell_2$ certificate, deploying data-dependent smoothing with the memory enhanced classifier yields significant improvement for the $\ell_1$ certified accuracy in all considered scenarios. }}
%         % , where the last column is the envelope.}
%         \label{fig:yang}
% \end{figure*}

\input{tables/l1}

==> Data-Dependent Randomized Smoothing-camera-ready/Sections/introduction.tex <==
\section{Introduction}
\label{introduction}
\blfootnote{* Equal contribution.}
\blfootnote{Correspondence to: motasem.alfarra@kaust.edu.sa, adel.bibi@eng.ox.ac.uk}
\footnote{Code: \href{https://github.com/MotasemAlfarra/Data_Dependent_Randomized_Smoothing}{https://github.com/MotasemAlfarra/DDRS.}}
Despite the success of Deep Neural Networks (DNNs) in various learning tasks \citep{krizhevsky2012imagenet,long2015fully}, they were shown to be vulnerable to small carefully crafted adversarial perturbations \citep{goodfellow2014explaining,szegedy2013intriguing}. For a DNN $f$ that correctly classifies an image $x$, $f$ can be fooled to produce an incorrect prediction for $x+\eta$ even when the adversary $\eta$ is so small that $x$ and $x+\eta$ are indistinguishable to the human eye. % Even worse, such adversaries, $\delta$, are in many cases easy to tailor with routines that are as simple as a single gradient ascent iteration of some loss function over the input \cite{goodfellow2014explaining}. This is of a critical concern particularly that DNNs are deployed in safety critical applications, \eg self driving cars, which can hinder their public trust. 
To circumvent this nuisance, there have been several works proposing heuristic training procedures to build networks that are \textit{robust} against such perturbations \citep{cisse2017parseval,madry2017towards}. However, many of these works provided a false sense of security as they were subsequently broken, \ie shown to be ineffective against stronger adversaries 
\input{figs/pull}
\citep{athalye2018obfuscated,tramer2020adaptive,uesato2018adversarial}. This has inspired researchers to develop networks that are \textit{certifiably robust}, \ie  networks that provably output constant predictions over a characterized region around every input. Among many certification methods, a probabilistic approach to certification called \textit{randomized smoothing} has demonstrated impressive state-of-the-art \textcolor{black}{certifiable robustness results \citep{cohen2019certified,lecuyer2019certified,li2018certified}.} In a nutshell, given an input $x$ and a base classifier $f$, \eg a DNN, randomized smoothing constructs a ``smooth classifier'' $g(x) = \mathbb{E}_{\epsilon\sim \mathcal{D}}\left[f(x+\epsilon)\right]$ such that, and under some choices of $\mathcal{D}$, $g(x) = g(x+\delta)~\forall \delta \in \mathcal{R}$. As such, $g$ is certifiable within the certification region $\mathcal{R}$ characterized by  $x$  and the smoothing distribution $\mathcal{D}$.  While there has been considerable progress in devising a notion of ``optimal'' smoothing distribution $\mathcal{D}$ for when $\mathcal{R}$ is characterized by an $\ell_p$ certificate \citep{yang2020randomized}, a common trait among all works in the literature is that the choice of $\mathcal{D}$ is independent from the input $x$. For example, one of the earliest works on randomized smoothing grants $\ell_2$ certificates under $\mathcal{D}=\mathcal{N}(0,\sigma^2 I)$, where $\sigma$ is a free parameter that is constant for all $x$ \citep{cohen2019certified}. That is to say, the classifier $f$ is smoothed to a classifier $g$ uniformly (same variance $\sigma^2$) over the entire input space of $x$. The choice of $\sigma$ used for certification is often set either arbitrarily or via cross validation to obtain best certification results \citep{salman2019provably}. We believe this is suboptimal and that $\sigma$ should vary with the input $x$ (data dependent), since using a fixed $\sigma$ may under-certify inputs (\ie the constructed smooth classifier $g$ produces smaller certification radii), which are far from the decision boundaries as exemplified by $x_1$ in Figure \ref{fig:pull_fig}. Moreover, this fixed $\sigma$ could be large for inputs $x$ close to the decision boundaries resulting in a smooth classifier $g$ that incorrectly classifies $x$ (refer to $x_3$ in Figure \ref{fig:pull_fig}).

In this paper, we aim to introduce more structure to the smoothing distribution $\mathcal{D}$ by rendering its parameters data dependent. That is to say, the base classifier $f$ is smoothed with a family of smoothing distributions to produce: $g(x) = \mathbb{E}_{\epsilon \sim \mathcal{N}(0,\textcolor{black}{\sigma^2_x}I)}\left[f(x+\epsilon)\right]$ 
\footnote{ The paper mainly focuses on Gaussian smoothing, but the idea holds for other parameterized distributions.}
. Note here that the variance of the Gaussian is now dependent on the data input $x$. Moreover, given that $\sigma_x$ varies with $x$, classical randomized smoothing based certification does not apply directly. We propose a simple memory-based approach to certify the resultant data dependent smooth classifier $g$. We show that \textcolor{black}{our memory-enhanced data dependent smooth classifier}
% this 
can boost certification performance of several randomized smoothing techniques. Our contributions can thus be summarized in three folds. (\textbf{i}) We propose a parameter free and generic framework that can easily turn several randomized smoothing techniques into their data dependent variants. In particular, given a network $f$ and an input $x$, we propose to optimize the smoothing distribution parameters for every $x$, \eg $\sigma^*_x$, so they maximize the certification radius. This choice of $\sigma^*_x$ is then used to smooth $f$ at $x$ and construct a smoothed classifier $g$. \textcolor{black}{Moreover, as the data dependent smooth classifier is not directly certifiable using \cite{cohen2019certified} MCMC approaches, we propose a memory-enhanced data dependent smooth classifier for certification.} (\textbf{ii}) We demonstrate the effectiveness of our \textcolor{black}{memory-enhanced data dependent smoothing}
% framework 
by showing that we can improve the certified accuracy of several models, specifically models trained with Gaussian augmentation (\textsc{Cohen}) \citep{cohen2019certified}, adversaries on the smoothed classifier (\textsc{SmoothAdv}) \citep{salman2019provably}, and radius regularization (\textsc{MACER}) \citep{zhai2020macer} \textit{without any model retraining}. We boost the certified accuracy of the best baseline by 5.4\% on CIFAR10 and by 2.8\% on ImageNet for $\ell_2$ perturbations with less than 0.5 (=127/255) ball radius. (\textbf{iii}) We show that incorporating the proposed data dependent smoothing in the training pipeline of \textsc{Cohen}, \textsc{SmoothAdv} and \textsc{MACER} can further boost results to get certified accuracies of 68.3\% on CIFAR10 and 64.2\% on ImageNet at $\ell_2$ perturbations less than 0.25.




==> Data-Dependent Randomized Smoothing-camera-ready/Sections/methodology.tex <==
\section{Data Dependent Smoothing}

% We first require some background on randomized smoothing before introducing our approach. Interested readers can follow \cite{cohen2019certified} for a more detailed description.

% We introduce our main technique for data dependent Gaussian smoothing. 


\subsection{Preliminaries and Notations}
% \vspace{-0.15cm}
% We consider the standard classification problem, 

Let $x \in \mathbb{R}^d$ and the labels $y \in \mathcal{Y} = \{1,\dots,k\}$ be the input-label pairs $(x,y)$ sampled from an unknown data distribution. Unless explicitly mentioned, we consider a classifier $f_\theta: \mathbb{R}^d \rightarrow \mathcal{P}(\mathcal{Y})$ parameterized by $\theta$ where $\mathcal{P}(\mathcal{Y})$ is a probability simplex over $k$ labels. We say that $f_\theta$ is $\ell_p^r$ certifiably accurate for an input $x$, if and only if, $\argmax_c f_\theta^c(x) = \argmax_c f_\theta^c(x+\delta) = y ~~\forall~ \|\delta\|_p \leq r$, where $f_\theta^c$ is the $c^{\text{th}}$ element of $f_\theta$. That is to say, the classifier correctly predicts the label of $x$  and enjoys a constant prediction for all perturbations $\delta$ that are in the $\ell_p$ ball of radius $r$ from $x$. As such, the overall $\ell_p^r$ certification accuracy is defined as the average certified accuracy over the data distribution. Following prior art \citep{cohen2019certified,salman2019provably,zhai2020macer}, we focus on $\ell_2^r$ certification. 

% We will denote hard and soft classifiers as $f_\theta: \mathbb{R}^d \rightarrow \mathcal{Y}$ and $\hat{f}_\theta: \mathbb{R}^d \rightarrow \mathcal{P}(\mathcal{Y})$, respectively, where $\mathcal{P}(\mathcal{Y})$ is a probability simplex in $\mathbb{R}^k$. We say that a hard classifier is $\ell_p^r$ certifiably accurate for an input $x$ if and only if $f_\theta(x) = f_\theta(x+\delta) = y, ~\forall~ \|\delta\|_p \leq r$ and equivalently $\argmax_c\hat{f}_\theta^c(x) = \argmax_c\hat{f}_\theta^c(x+\delta) = y, ~\forall~ \|\delta\|_p \leq r$ for soft classifiers, where $\hat{f}_\theta^c$ is the $c^{\text{th}}$ element of $\hat{f}_\theta$. That is to say, the classifier correctly predicts the label of $x$  and enjoys a constant prediction for all perturbations $\delta$ that are in the $\ell_p$ ball of radius $r$ from $x$. As such, the overall $\ell_p^r$ certification accuracy is defined as the average certified accuracy over the data distribution. In this paper and following previous works \cite{\textsc{Cohen}2019certified,salman2019provably,zhai2020\textsc{MACER}}, we focus on $\ell_2^r$ certification.  


% \[g_\theta(x) = \argmax_{c}~ \mathbb{P}_\epsilon \left(f_\theta (x+\epsilon)=c\right).\]
% \begin{definition}
% \label{def_hard_classifier}
% For any $\sigma > 0$, the smoothed classifier of $f_\theta$ is defined as follows with $\epsilon \sim \mathcal{N}(0,\sigma^2I)$:
% \begin{equation}
% \label{eq:def_smoothed_class}
% \begin{aligned}
%     g_\theta(x) = \argmax_{c}~ \mathbb{P}_\epsilon \left(f_\theta (x+\epsilon)=c\right).
% \end{aligned}
% \end{equation}
% \end{definition}
% It is generally difficult to use $g_\theta$ for prediction as that requires the output density of an arbitrary $f_\theta$ under Gaussian input. However, \cite{\textsc{Cohen}2019certified} proposed a Monte Carlo algorithm that succeeds in predicting the class of $x$ by $g_\theta$ with high probability.

\subsection{Overview of Randomized Smoothing}
% \vspace{-0.15cm}
% Randomized smoothing constructs a smoothed classifier $g_\theta$ from an arbitrary classifier $f_\theta$ assigning the most likely class to be predicted by $f_\theta$ if inputs were subjected to isotropic Gaussian perturbations. 
Randomized smoothing constructs a certifiable classifier $g_\theta$ by smoothing a base classifier $f_\theta$. For any $\sigma > 0$, the smooth classifier is defined as: $g_\theta(x) = \mathbb{E}_{\epsilon \sim \mathcal{N}(0,\sigma^2I)} \left[f_\theta (x+\epsilon)\right]$. 
% More importantly, \cite{\textsc{Cohen}2019certified} presented a tight certification radius within which the smoothed classifier $g_\theta$ is certifiable. 
Let $g_\theta$ predict label $c_A$ for input $x$ with some confidence, \ie $\mathbb{E}_\epsilon[f^{c_A}_\theta(x+\epsilon)] = p_A \ge p_B = \max_{c \neq c_A} \mathbb{E}_\epsilon[f^c_\theta(x+\epsilon)]$, then, $g_\theta$ is certifiably robust at $x$ with certification radius:
\begin{equation}
\begin{aligned}
    \label{eq:certification_radius}
        R =  \frac{\sigma}{2} \left(\Phi^{-1}(p_A) - \Phi^{-1}(p_B)\right).
\end{aligned}
\end{equation}
Here,  $g(x+\delta) = g(x)~\forall \|\delta\|_2 \leq R$, where $\Phi$ is the CDF of the standard Gaussian. 
% We refer to $R$ throughout as the certification radius. 



\subsection{Robustness-Accuracy Trade-off}
% \vspace{-0.15cm}
Note that Equation \ref{eq:certification_radius} holds regardless of the prediction $c_A$ made by the smooth classifier $g_\theta$. This suggests that one can perhaps improve the robustness of $g_\theta$, \ie increase certification radius $R$ where $g_\theta$ is constant, by increasing the hyper parameter $\sigma$ in Equation \ref{eq:certification_radius}. However, to reason about $\ell_2^r$ certification accuracy, it is not enough to increase the certification radius $R$, as this requires $c_A$ to be the correct prediction for $x$ by $g_\theta$. This reveals the robustness-accuracy trade-off as one cannot improve $\ell_2^r$ certified accuracy by only increasing  the certification radius $R$ (robustness) through the increase in $\sigma$. This is because it comes at the expense of requiring a classifier $g_\theta$ that correctly classifies $x$ with correct label $y$ under large Gaussian perturbations (accuracy). As such, the following inequality should hold $\mathbb{E}_\epsilon[f^{\textcolor{red}{y}}_\theta(x+\epsilon)] \ge p_A \ge p_B \ge \max_{c \neq \textcolor{red}{y}} \mathbb{E}_\epsilon[f^c(x+\epsilon)]$. 

% This establishes the role of $\sigma$ in trading off robustness with accuracy.

% the certification radius $R$


% The robustness-accuracy trade-off now comes as one can not improve the $\ell_2^r$ certified accuracy by increasing $\sigma$ as that comes at the expense of requiring a classifier $g_\theta$ that correctly classifies $x$ with correct label $y$ under large Gaussian perturbations (accuracy), \ie the following inequality holds $\mathbb{P}_\epsilon(f(x+\epsilon) = \textcolor{red}{y}) \ge p_A \ge p_B \ge \max_{c \neq \textcolor{red}{y}} \mathbb{P}_\epsilon(f(x+\epsilon) = c)$.

% This reveals the robustness-accuracy trade-off. O

% ne cannot improve the $\ell_2^r$ certification radius (robustness) by increasing $\sigma$ as that comes at the expense of requiring a classifier $g_\theta$ correctly classifying $x$ with correct label $y$ under large Gaussian perturbations (accuracy), \ie the following inequality holds $\mathbb{P}_\epsilon(f(x+\epsilon) = \textcolor{red}{y}) \ge p_A \ge p_B \ge \max_{c \neq \textcolor{red}{y}} \mathbb{P}_\epsilon(f(x+\epsilon) = c)$ \BG{this sentence is too long; break it up into smaller pieces}. This establishes the role of $\sigma$ in trading off robustness with accuracy.


\subsection{Data Dependent Smoothing for Certification}
% \vspace{-0.15cm}

The certification region $\mathcal{R} = \{\delta : \|\delta\|_2 \leq R\}$ at an input $x$ is fully characterized by the classifier $f_\theta$ and the standard deviation of the Gaussian distribution $\sigma$. Moreover, for a given $f_\theta$, the certification region $\mathcal{R}$ varies at different $x$, when $\sigma$ is fixed, due to the nonlinear dependence of the prediction gap
% \vspace{-0.5cm}
$\Phi^{-1}(p_A(x;\sigma)) - \Phi^{-1}(p_B(x;\sigma))$ on $x$. This hints that, for a given $f_\theta$, different inputs $x$ may enjoy a different optimal $
\sigma^*_x$ that maximizes the certification region. To see this, consider the three inputs $x_1$, $x_2$ and $x_3$ all correctly classified  by the binary classifier $f_\theta$ as $\mathcal{C}_1$ in Figure \ref{fig:pull_fig}. Using a fixed $\sigma$ to smooth the predictions of $f_\theta$, \ie predict with $g_\theta$, reveals that inputs, depending on how close they are from the decision boundaries, can enjoy different levels of smoothing without affecting the prediction of $g_\theta$. For instance, as shown in Figure \ref{fig:pull_fig} for constant $\sigma$, the input far from the decision boundary $x_1$ could have still been classified correctly with similarly large prediction gap even if $f_\theta$ were to be smoothed with a larger $\sigma$. This indicates that perhaps the certification radius at $x_1$ could have been enlarged with a larger smoothing $\sigma$. As for $x_2$, we can observe that while the prediction under this choice of $\sigma$ by $g_\theta$ is still correct, the prediction gap $\Phi^{-1}(p_A(x;\sigma)) - \Phi^{-1}(p_B(x;\sigma))$ drops, due to having more Gaussian samples fall in the $\mathcal{C}_2$ region. Thus, a different choice of $\sigma$ could have been used to trade-off the drop in prediction gap and certification radius.
% \begin{wrapfigure}{r}{0.5\textwidth}
% % \vspace{-0.25cm}
% \begin{minipage}
% \begin{algorithmic}
\begin{algorithm}[t]
  \DontPrintSemicolon
  \SetKwFunction{FMain}{\small OptimizeSigma}
  \SetKwProg{Fn}{Function}{:}{}
  \Fn{\FMain{$f_\theta$, $x$, $\alpha$, $\sigma_0$, $n$}}{
  \textbf{Initialize:} $\sigma_x^0 \gets \sigma_0$, $K$ \;
     \For{$k = 0 \dots K-1$ }{
     sample $\hat{\epsilon}_1,\dots \hat{\epsilon}_n \sim \mathcal N(0,I)$ \;
     $ \psi(\sigma^{k}_x) = \frac{1}{n} \sum_{i=1}^n f_\theta(x + \sigma^{k}_x\hat{\epsilon}_i)$\;
     $E_A(\sigma_x^k) = \max_c \psi^c$; $y_A = \argmax_c \psi^c$;\;
     $E_B(\sigma_x^k) = \max_{c \neq y_A} \psi^c$ \;
     $R(\sigma_x^k) =  \frac{\sigma^{k}_x}{2}\left(\Phi^{-1}(E_A) - \Phi^{-1}(E_B)\right)$ \;
    $\sigma^{k+1}_x \gets \sigma^{k}_x + \alpha \nabla_{\sigma_x^k}R(\sigma^{k}_x)$
     }
     $\sigma^*_x \leftarrow \sigma^K_x$ \;
        \KwRet $\sigma^*_x$ \; }
  \caption{ Data Dependent Certification}\label{alg:RS_DS}
% \vspace{-0.6cm}
\end{algorithm}
% \end{algorithmic}
% \end{minipage}
% \end{wrapfigure}
Last, for the input $x_3$ that is very close to the decision boundary, the sub optimal choice of $\sigma$ (too large for $x_3$) could result in an incorrect prediction by $g_\theta$. Despite the observations that $\sigma$ plays a significant role in $\ell_2^r$ certification accuracy, certification methods generally (\textbf{i})  choose $\sigma$ arbitrarily and (\textbf{ii}) set it to be constant for all $x$. Based on this observation, for a given smooth classifier with a specific $\sigma_0$, where $\sigma_0$ can be zero reducing the smooth classifier to $f_\theta$, we seek to construct another smooth classifier with parameter $\sigma_x^*$ for every input $x$ such that: (\textbf{i}) the prediction of both smooth classifiers (smoothing with $\sigma_0$ and $\sigma_x^*$) is identical for all $x$. (\textbf{ii}) The certification radius of the new smooth classifier at every $x$ is maximized. 
% If both conditions (\textbf{i}) and (\textbf{ii}) hold for every input $x$, then the new smooth classifier with $\sigma_x^*$ for every corresponding $x$ will enjoy a larger certification radius at every $x$ compared to the one smoothed with $\sigma_0$ while both retain the same predictions.
% will enjoy a certified accuracy $\ell_2^r$ that is at least equal to the $\ell_2^r$ certified accuracy of the classifier smoothed with $\sigma_0$. 
To construct a classifier smoothed with $\sigma_x^*$ enjoying the two previous properties, let $c_A$ be the prediction under $\sigma_0$ smoothing, \ie $c_A = \argmax_c \mathbb{E}_{\epsilon\sim\mathcal{N}(0, \sigma_0I)}[f^c(x+\epsilon)]$. We maximize $R$ in Equation \ref{eq:certification_radius} over $\sigma$ for every $x$ by solving:
% \vspace{-0.65cm}
\begin{equation}
\label{eq:our_objective}
\begin{aligned}
    \sigma^*_x =&\argmax_{\sigma} ~\frac{\sigma}{2} \Bigg(\Phi^{-1}\left( \mathbb{E}_{\epsilon \sim \mathcal{N}(0,\sigma^2I)}[f_\theta^{c_A}(x+\epsilon)]\right)  \\ \,\, - \,\, & \Phi^{-1}\left(\max_{c \neq c_A} \mathbb{E}_{\epsilon \sim \mathcal{N}(0,\sigma^2I)}[f_\theta^c(x+\epsilon)]\right) \Bigg).
\end{aligned}
\end{equation}
Since $\Phi^{-1}$ is a strictly increasing function, it is important to note that solving Equation \ref{eq:our_objective} for a fixed $c_A$ can at worst yield a smooth classifier of an identical radius to when the classifier is smoothed with $\sigma_0$ both predicting $c_A$ for $x$. 

\noindent \textbf{Solver}.
While our proposed Objective \ref{eq:our_objective} has a similar form to the \textsc{MACER} regularizer \citep{zhai2020macer} used during training, ours differs in that we optimize $\sigma$ for every $x$ and not the network parameters $\theta$, which are fixed here. A natural solver for \ref{eq:our_objective} is stochastic gradient ascent with the expectation approximated with $n$ Monte Carlo samples. As such, the gradient of the objective at the $k^{\text{th}}$ iteration  will be approximated as follows: $% \vspace{-0.15cm}
% \begin{align*}
   \nabla_{\sigma^k} \frac{\sigma^k}{2}\left[ \Phi^{-1}\left(\gamma^{c_A}(\sigma^k)\right) - \Phi^{-1}\left(\max_{c \neq c_A} \gamma^c(\sigma^k)\right)\right],
% \end{align*}$
$ where $\gamma^c(\sigma^k) = \frac{1}{n}\sum_{i=1}^n f^c(x+\epsilon_i)$ for $\epsilon_1, \dots, \epsilon_n \sim \mathcal{N}(0,(\sigma^k)^2I)$. However, this estimation of the gradient suffers from high variance due to the dependence of the expectation on the optimization variable $\sigma$ that parameterizes the smoothing distribution $\mathcal{N}(0,\sigma^2 I)$ \citep{williams1992simple}. %Interestingly, one can observe that our objective is very similar to the Evidence Lower Bound (ELBO) objective used to train variational auto encoders (VAEs) \cite{kingma2014auto,rezende2014stochastic}. The similarities between \eqref{eq:our_objective} and ELBO are in the dependence of the expectation on the variables of optimization. 
To alleviate this, we use the \textit{reparameterization trick} suggested by \cite{kingma2014auto,rezende2014stochastic} to compute a lower variance gradient estimate for our Objective \ref{eq:our_objective}. In particular, with the change of variable $\epsilon = \sigma \hat{\epsilon}$ where $\hat{\epsilon} \sim \mathcal{N}(0,I)$, Objective \ref{eq:our_objective} is \textit{equivalent to}:
% \vspace{-0.15cm}
\begin{equation}
\label{eq:our_objective_v2}
\begin{aligned}
    \sigma^*_x =&\argmax_{\sigma} \frac{\sigma}{2} \Bigg(\Phi^{-1}
    \left(\mathbb{E}_{\hat{\epsilon}\sim \mathcal{N}(0,I)}[f_\theta^{c_A}(x+\sigma \hat{\epsilon})]\right) - \\ & \Phi^{-1}\left(\max_{c \neq c_A} \mathbb{E}_{\hat{\epsilon}\sim \mathcal{N}(0,I)}[f_\theta^c(x+\sigma\hat{\epsilon})]\right)\Bigg)
\end{aligned}
\end{equation}
\noindent Note that, unlike before, the expectation over the distribution $\hat{\epsilon} \sim \mathcal{N} (0,I)$ no longer depends on the optimization variable $\sigma$. This allows the gradient of \ref{eq:our_objective_v2} to enjoy a lower variance compared to the gradient of \ref{eq:our_objective} \citep{kingma2014auto,rezende2014stochastic}. Algorithm \ref{alg:RS_DS} summarizes the updates for optimizing $\sigma$ for each $x$ by solving \ref{eq:our_objective_v2} with $K$ steps of stochastic gradient ascent. It is worthwhile to mention that the function \texttt{OptimizeSigma} in Algorithm \ref{alg:RS_DS} is agnostic of the choice of architecture $f_\theta$ and of the training procedure that constructed $f_\theta$. 


% \textcolor{red}{Once $\sigma_x^*$ is attained by \texttt{OptimizeSigma} for a given model $f_\theta$, we certify the smoothed classifier $g_\theta$ under this $\sigma_x^*$ using the Monte Carlo algorithms proposed by \cite{cohen2019certified}.}

% Empirically, we demonstrate the effectiveness of the proposed algorithm by certifying pre-trained models with (i) Gaussian augmentation (\textsc{Cohen}) \cite{cohen2019certified}, (ii) adversarially trained smoothed classifiers (\textsc{SmoothAdv}) \cite{salman2019provably}, and (iii) \textsc{MACER} \cite{zhai2020macer}, where $\sigma^*_x$ is used for each $x$. 



\begin{figure*}[t]
    \centering
    % \includegraphics[width=\textwidth]{ICLR22/new_figures/post_certificate.png}
    \includegraphics[width=\textwidth]{figures/post_certificate_2.png}
    \caption{ \textbf{Memory-based certification of the data dependent classifier.} Given a memory of an input $x_1$ with a certified region $\mathcal{R}_1$ and another input $x_2$ with a certified region $\mathcal{R}_2$. Three scenarios could arise where $\mathcal{R}_1$ and $\mathcal{R}_2$ intersect. \textbf{Left}: The certified regions intersect while both $x_1$ and $x_2$ share the same prediction. In this case, $x_2$ along with its certified region are directly added to memory. \textbf{Middle}: $x_2$ lies inside $\mathcal{R}_1$ with a different prediction from $x_1$. In this case, $x_2$ is predicted with the same prediction as $x_1$ and  added to memory along with the largest subset of $\mathcal{R}_2$ that is within $\mathcal{R}_1$. \textbf{Right}: $x_2$ lies outside the $\mathcal{R}_1$ with a different prediction from $x_1$ In this case, $x_2$ with its prediction are added to memory along with the largest certified region in $\mathcal{R}_2$ not intersecting with $\mathcal{R}_1$.}
    \label{fig:memory-based-algorithm}
    % \vspace{-0.50cm}
\end{figure*}


\subsection{Memory-Based Certification for Data Dependent Classifiers}\label{sec:memory-algorithm}

Unlike previous approaches where $\sigma$ is constant for all inputs, the data dependent classifier $g_\theta$ with varying $\sigma$ per input can not be directly certified by the classical Monte Carlo algorithms proposed by \cite{cohen2019certified}. This is since the data dependent classifier $g_\theta$ does not enjoy a constant $\sigma$ within the given certification region, \ie $g_\theta$ tailors a new $\sigma_x$ for every input $x$ including within the certified region of $x$. Informally, let $R(\sigma_{x_1}^*)$ be the radius of certification at $x_1$ granted by the data dependent classifier $g_\theta$. The data dependent classifier \textit{does not guarantee} that there \textit{can not exist} $x_2$ within the region of certification of $x_1$, \ie $\|x_1 - x_2\|_2 \leq R(\sigma_{x_1}^*)$, where $g_\theta$ with $\sigma_{x_2}^*$ predicts  $x_2$ differently from $x_1$ breaking the soundness of certification. 
% \begin{wrapfigure}{r}{0.60\textwidth}\vspace{-0.15cm}
% \begin{minipage}{0.60\textwidth}
\begin{algorithm}[t]
% \small
  \DontPrintSemicolon
  \SetKwFunction{FMain}{TrainBatch}
  \SetKwProg{Fn}{Function}{:}{}
  \Fn{\FMain{$f_\theta$, $\{x_i,y_i\}_{i=1}^B$, $\{ \sigma_{x_i}\}_{i=1}^B$, $\alpha$, $n$}}{
 \For{$i=1, \dots, B$}{
   $\sigma^*_{x_i} = \texttt{\small OptimizeSigma}(f_\theta, x_i, \alpha, \sigma_{x_i}, n)$
 }
 \texttt{\small TrainFunction} $\left(\{x_i,y_i\}_{i=1}^B, \{\sigma^*_{x_i}\}_{i=1}^B\right)$ 
  \tcp{\small any training routine e.g. \textsc{MACER}}
 }
   \caption{ Training with Data Dependent $\sigma_{x_i}$} \label{alg:DS_DS}
\end{algorithm}
% \end{minipage}
% \vspace{-0.50cm}
% \end{wrapfigure} 
To circumvent this problem, we propose a memory-based procedure to certifying our proposed data dependent classifier. Let $\{x_i\}_{i=1}^N$ be a set of previously predicted inputs and $\{\mathcal{C}_i\}_{i=1}^N$ be their corresponding predictions with mutually exclusive $\ell_2$ certified regions $\mathcal{R}_i$ for differently predicted inputs, \ie $\mathcal{R}_i \cap \mathcal{R}_j = \emptyset ~\forall i\neq j, \mathcal{C}_i \neq \mathcal{C}_j$. Let $x_{N+1}$ be a new input with a certified region $\mathcal{R}_{N+1}$ computed by the Monte Carlo algorithms of \cite{cohen2019certified} for the data dependent classifier $g_\theta$ with prediction $\mathcal{C}_{N+1}$. If there exists an $i$ such that $\mathcal{R}_{N+1} \cap \mathcal{R}_i \neq \emptyset$,  $x_{N+1} \in \mathcal{R}_i$, and $\mathcal{C}_{N+1} \neq \mathcal{C}_i$, we adjust the prediction of the data dependent classifier $g_\theta$ to be $\mathcal{C}_i$ and update $\mathcal{R}_{N+1}$ to be the largest subset of $\mathcal{R}_{N+1}$ that is a subset of $\mathcal{R}_i$ (see middle example in Figure \ref{fig:memory-based-algorithm}). %We then add the $x_{N+1}$, $\mathcal{C}_{N+1}$, and $\tilde{\mathcal{R}}_{N+1}$ to memory. 
On the other hand, if $\mathcal{R}_{N+1} \cap \mathcal{R}_i \neq \emptyset$, $x_{N+1} \notin \mathcal{R}_i$, and that $\mathcal{C}_{N+1} \neq \mathcal{C}_i$, we update $\mathcal{R}_{N+1}$ to be the largest subset of $\mathcal{R}_{N+1}$ not intersecting with $\mathcal{R}_i$ (see right example in Figure \ref{fig:memory-based-algorithm}). We perform the previous operations for all elements in the memory and add $x_{N+1}, \mathcal{C}_{N+1}, 
\mathcal{R}_{N+1}$ to memory. The aforementioned procedure grants a sound certification for the data dependent classifier preventing by construction overlapping certified regions with different predictions.% $\mathcal{C}$ as $\mathcal{C}_{N+1}$  by the Monte Carlo algorithms of \cite{cohen2019certified}, if $x_{N+1} \in \mathcal{R}_i$ where $\mathcal{C}_{}$
% we adjust the prediction of the data dependent classifier to be $\mathcal{C}_i$ if $x_{N+1} \in \mathcal{R}_i$ and $\mathcal$. Otherwise, \ie $x_{N+1} \notin \mathcal{R}_i \forall i$, we predict with our proposed data dependent classifier and compute the certification region $\mathcal{R}_{N+1}$. We then update the memory with the new input $x_{N+1}$ and its certified region $\mathcal{R}_{N+1}$ while satisfying the mutually exclusive property for differently predicted inputs, \ie $\mathcal{R}_i \cap \mathcal{R}_j = \emptyset, \forall i\neq j, c_i \neq j$. To do so, two cases arise that we summarize in the middle and right examples of Figure \ref{fig:memory-based-algorithm}. In the first case, middle example of Figure \ref{fig:memory-based-algorithm}, we adjust the prediction of the data dependent classifier to $\mathcal{C}_i$ and find the largest subset of $\mathcal{R}_{N+1}$ that is within $\mathcal{R}_1$ and then add it to memory. The other case, right example in Figure \ref{fig:memory-based-algorithm}, where $x_{N+1} \notin \mathcal{R}_1$ with $\mathcal{C}_i \neq \mathcal{C}_{N+1}$, we find the largest subset of $\mathcal{R}_{N+1}$ not intersecting with $\mathcal{R}_1$
% or reduce the certified region to the largest overlapping radius. We then certify the aforementioned data dependent classifier using the Monte Carlo algorithms proposed by \cite{cohen2019certified}. 
While the memory-based certification is essential for a sound certification, empirically, we never found in any of the later experiments a case where two inputs predicted differently suffer from intersecting certified regions. That is to say \textcolor{black}{while our sound certificate works on the memory-enhanced data dependent smooth classifier, we found that} the certified \textcolor{black}{radius of}
% regions in
the memory \textcolor{black}{classifier} for every input is the \textcolor{black}{radius}
% regions 
granted by the Monte Carlo certificates of \cite{cohen2019certified} for 
the data dependent classifier. \textcolor{black}{Therefore and throughout, we refer to the memory-enhanced data dependent smooth classifier and data dependent smooth classifier interchangeably.}
We elaborate more on this and provide an algorithm in the \textbf{Appendix}.


% Figure \ref{fig:memory-based-algorithm} summarizes the three cases in which an overlap happens where our memory based procedure corrects the certified radius alone (Right) or adjusts the predicted label as well (middle).





% $x_{N+1}$ to we have that



% To circumvent this problem, we propose a memory based procedure that corrects the data-dependent certified radii such that we guarantee non-overlapping certified regions between differently predicted samples. In a nutshell at test time, as a new sample $x_i$ approaches, we check if there is an overlap between its certified region and any certified region of a differently predicted sample saved in memory. If that is the case, then we adjust the certified radius of the new sample such that no overlap happens. We then save the sample along with its optimal smoothing parameter, its predicted label, and its certified radius in memory. Figure \ref{fig:memory-based-algorithm} summarizes the three cases in which an overlap happens where our memory based procedure corrects the certified radius alone (Right) or adjusts the predicted label as well (middle).




\subsection{Training with Data Dependent Smoothing}
% \vspace{-0.15cm}
Models that enjoy a large $\ell_2^r$ certification accuracy under the randomized smoothing framework need to enjoy a large certification radius $R$ in Equation \ref{eq:certification_radius} for all $x$ and be able to correctly classify inputs corrupted with Gaussian noise, \ie $g_\theta(x) = y$. While there are several approaches to train $f_\theta$ (or directly $g_\theta$) so as to output correct predictions for inputs corrupted with noise sampled from $\mathcal{N}(0,\sigma^2 I)$, all existing works fix $\sigma$ for all inputs during training. We are interested in complementing these approaches with smoothing distributions that are data dependent. As such, we can employ the training procedure of these approaches but with $\sigma^*_x$ computed by \texttt{OptimizeSigma}. Algorithm \ref{alg:DS_DS} summarizes this proposed training pipeline. The function \texttt{TrainFunction} proceeds by performing backpropagation using any training scheme, given the estimated $\sigma^*_{x_i}$ for each $x_i$. We note that whenever Algorithm \ref{alg:DS_DS} is used, we initialize $\sigma_{x_i}$ at each epoch with $\sigma^*_{x_i}$ computed at the previous epoch. Since \textsc{Cohen}, \textsc{SmoothAdv} and \textsc{MACER} are among the most popular approaches that embed randomized smoothing certificates as part of the training routine,  \texttt{TrainFunction} refers here to any of these three training methods. Empirically, we show that we can boost all three methods even further when models are trained with Algorithm \ref{alg:DS_DS}.




% \textcolor{red}{Motasem: I think we should add the paragraph here}






% \begin{algorithm}[t]
%   \DontPrintSemicolon
%   \SetKwFunction{FMain}{Train}
%   \SetKwProg{Fn}{Function}{:}{}
%   \Fn{\FMain{$f_\theta$, $\{x_i,y_i\}_{i=1}^B$, $\alpha$, $K$, $M$, $S$, $\sigma_0$}}{
%   \textbf{Initialize:} $\sigma^*_{x_i} \gets \sigma_0\,\, \forall i\in\{1,\dots,B\}$ \\
%  \For{$j=1,\dots M$}{
%  \If{$j \geq S$}{
%  \For{$i=1, \dots, B$}{
%   $\sigma^*_{x_i} = \texttt{OptimizeSigma}(f_\theta, x_i, \alpha, \sigma^*_{x_i}, K)$
%  }}
%  \texttt{TrainFunction} $\left(\{x_i,y_i\}_{i=1}^n, \{\sigma^*_{x_i}\}_{i=1}^n\right)$  \;
%  }}
%   \caption{Training with Data Dependent Smoothing} \label{alg:RS_DS}
% \end{algorithm}


% \begin{algorithm}[t]
% \SetAlgoLined
% \textbf{Inputs:} Network $f_\theta$, batch size B, epochs, step size $\alpha$, number of optimization iterations $K$\\
%  \For{$j=1, \dots, \text{epochs}$ }{
%  \For{$i=1, \dots, B$}{
%   $\sigma^*_{x_i} = \texttt{OptimizeSigma}(f_\theta, x_i, \alpha, \sigma_{x_i}, K)$

%  Train with $x_i$ and $\mathcal N(0,\sigma^*_{x_i}I)$ \;
% %  Sample $\epsilon \sim \mathcal N(0,\sigma(x_i)I)$ \;
%  }}
%  \textbf{Output:} model parameters $\theta$
%  \caption{Training with Data Dependent Smoothing} \label{alg:DS_DS}
% \end{algorithm}


% To that regard, we are


% In general, for correctly classified inputs by $g_\theta$, one would generally be interested in doing so with as large $\sigma$ as possible as that can increase the certification radius.



% resulted in incorrect predictions

% ote that one can view the predictions by $g_\theta$ as th average prediction

% could have enjoyed a larger certification radius by $g_\theta$ certified by a larger radius $\sigma$ without changing the correct prediction of $g_\theta$

% far  is far from the decision boundary could have been certified by a larger radius $\sigma$ without changing the correct prediction of $g_\theta$

% points that are close to the decision boundary $x_2$ may have their correct predictions affected much more that points far away from decision boundary, e.g. $x_1$.




% In the first case, figure \ref{fig:pull_fig}, the classifier $g_\theta$ smooths the predictions over all points by the same amount $\sigma$. Note $g_\theta$, can be viewed as the average prediction of $f_\theta$ under Gaussian perturbations, is the average 

% both classified correctly by the binary classifier $f_\theta$ shown in Figure \textcolor{red}{x}. It is to be observed that for the sample $x_1$, which is far away from the decision boundary, the prediction of the classifier $g_\theta$ is less sensitive to the increase in $\sigma$ as compared to the prediction of $g_\theta$ at $x_2$ that is close to the decision boundary. 



==> Data-Dependent Randomized Smoothing-camera-ready/Sections/related_work.tex <==
\section{Related Work}
\label{related_work}

\textbf{Certified Defenses.} Certified defenses aim to guarantee that an adversary does not exist in a certain region around a given input. Certified defenses can be divided into exact \citep{cheng2017maximum,lomuscio2017approach,huang2017safety,ehlers2017formal} and relaxed certification \citep{salman2019convex, wong2018provable}. Generally, exact certification suffers from poor scalability with networks that are at most 3 hidden layers deep \citep{tjeng2017evaluating}. On the other hand, relaxed methods resolve this issue by aiming at finding an upper bound to the worst adversarial loss over all possible bounded perturbations around a given input \citep{weng2018towards}. However, the latter is too expensive for any mixed certification-training routine. 


\textbf{Randomized Smoothing.} %Randomized smoothing is a recent probabilistic approach to certification. 
The earliest work on randomized smoothing \citep{lecuyer2019certified} was from a differential privacy  perspective, where it was demonstrated that adding Laplacian noise enjoys an $\ell_1$ certification radius in which the average classifier prediction under this noise is constant. This work was later followed by the tight $\ell_2$ certificate radius for Gaussian smoothing \citep{cohen2019certified}. Since then, there has been a body of work on randomized smoothing with empirical defenses \citep{salman2019provably} to certify black box classifiers \citep{salman2020black}. Other works derived certification guarantees for $\ell_1$ bounded \citep{teng2019ell_1}, $\ell_\infty$ bounded \citep{zhang2019filling}, and $\ell_0$ bounded \citep{levine2020robustness} perturbations. Even more recently, a novel framework that finds the optimal smoothing distribution for a given $\ell_p$ norm \citep{yang2020randomized} was proposed showing state-of-art certification results on $\ell_1$ perturbations. We deviate from the common literature by introducing the notion of smoothing, particularly Gaussian smoothing for $\ell_2$ perturbations, which varies depending on the input. In particular, since an input $x$ that is far from the decision boundaries should tolerate larger smoothing (and equivalently have a larger certification radius) as compared to inputs closer to these boundaries, we optimize for the amount of smoothing per input (specifically $\sigma_x$) that maximizes the certification radius. This proposed process is denoted as \emph{data dependent smoothing} where we provide a procedure for certifying the resultant smooth classifier.


% \BG{similar to the intro, we have to give a clear justification of  why we expect that making it data dependent will be better}

==> Data-Dependent Randomized Smoothing-camera-ready/figs/Cohen.tex <==
\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar10/RS/all_1.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar10/RS/all_2.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar10/RS/all_3.png}
     \end{subfigure}
      \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/cifar10/RS/all_4.png}
     \end{subfigure}
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/imagenet/RS/all_1.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/imagenet/RS/all_2.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/imagenet/RS/all_3.png}
     \end{subfigure}
      \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/imagenet/RS/all_4.png}
     \end{subfigure}
    %  \vspace{-0.25cm}
     \caption{\textbf{Certified accuracy comparison against $\text{Cohen}$ per radius per $\sigma$.} We compare $\text{Cohen}$ against our data dependent certification $\text{Cohen-DS}$ and when data dependency is incorporated in both training and certification $\text{Cohen-DS}^2$ for several $\sigma$. The value of $\sigma$ shown for our models in the legend refers to the optimization initialization $\sigma_0$ in Algorithm \ref{alg:RS_DS}. We show CIFAR10 and ImageNet results in first and second rows, respectively, where the last column is the envelope.}
        \label{fig:GA}
        % \vspace{-0.15cm}
\end{figure*}







==> Data-Dependent Randomized Smoothing-camera-ready/figs/MACER.tex <==

\begin{figure*}[t]
     \centering
    %  \begin{subfigure}[b]{0.24\textwidth}
    %      \centering
         \includegraphics[width=0.24\textwidth]{  figures/cifar10/MACER/all_1.png}
    %  \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{0.24\textwidth}
    %      \centering
         \includegraphics[width=0.24\textwidth]{  figures/cifar10/MACER/all_2.png}
    %  \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{0.24\textwidth}
    %      \centering
         \includegraphics[width=0.24\textwidth]{  figures/cifar10/MACER/all_3.png}
    %  \end{subfigure}
    %   \begin{subfigure}[b]{0.24\textwidth}
    %      \centering
         \includegraphics[width=0.24\textwidth]{  figures/cifar10/MACER/all_4.png}
    %  \end{subfigure}
    %  \vspace{-0.25cm}
     \caption{\textbf{Certified accuracy comparison against $\text{MACER}$ per radius per $\sigma$.} We compare $\text{MACER}$ against
    %  our data dependent certification 
     $\text{MACER-DS}$ and 
    %  when data dependency is incorporated in both training and certification 
     $\text{MACER-DS}^2$
     for several $\sigma$ 
     on CIFAR10
     with the last column showing the envelope.}
        \label{fig:MACER}
        \vspace{-0.15cm}
\end{figure*}

==> Data-Dependent Randomized Smoothing-camera-ready/figs/SmoothAdv.tex <==

\begin{figure*}[t]
     \centering
    %  \begin{subfigure}[b]{0.24\textwidth}
    %      \centering
         \includegraphics[width=0.24\textwidth]{  figures/cifar10/advsmooth/all_1.png}
    %  \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{0.24\textwidth}
        %  \centering
         \includegraphics[width=0.24\textwidth]{  figures/cifar10/advsmooth/all_2.png}
    %  \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{0.24\textwidth}
    %      \centering
         \includegraphics[width=0.24\textwidth]{  figures/cifar10/advsmooth/all_3.png}
    %  \end{subfigure}
    %   \begin{subfigure}[b]{0.24\textwidth}
    %      \centering
         \includegraphics[width=0.24\textwidth]{  figures/cifar10/advsmooth/all_4.png}
    %  \end{subfigure}
    %       \begin{subfigure}[b]{0.24\textwidth}
    %      \centering
         \includegraphics[width=0.24\textwidth]{  figures/imagenet/advsmooth/all_1.png}
    %  \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{0.24\textwidth}
        %  \centering
         \includegraphics[width=0.24\textwidth]{  figures/imagenet/advsmooth/all_2.png}
    %  \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{0.24\textwidth}
    %      \centering
         \includegraphics[width=0.24\textwidth]{  figures/imagenet/advsmooth/all_3.png}
    %  \end{subfigure}
    %   \begin{subfigure}[b]{0.24\textwidth}
    %      \centering
         \includegraphics[width=0.24\textwidth]{  figures/imagenet/advsmooth/all_4.png}
    %  \end{subfigure}
    %  \vspace{-0.25cm}
        \caption{\textbf{Certified accuracy comparison against $\text{SmoothAdv}$ per radius per $\sigma$.} We compare $\text{SmoothAdv}$ against
        % our data dependent certification
        $\text{SmoothAdv-DS}$ and
        % and when data dependency is incorporated in both training and certification
        $\text{SmoothAdv-DS}^2$.
        % for several $\sigma$. 
        We show CIFAR10 and ImageNet results in first and second rows, respectively.}
        % , where the last column is the envelope.}
        \label{fig:SmoothAdv}
\end{figure*}

==> Data-Dependent Randomized Smoothing-camera-ready/figs/iteration_ablation.tex <==
\begin{figure}[t]\vspace{-0.2cm}
\centerline{
     \includegraphics[width=0.24\textwidth]{figures/iterations/CIFAR10_Adv_smooth_DS_DS_sigma_012.png}\hfill
    \includegraphics[width=0.24\textwidth]{figures/iterations/ImageNet_Adv_smooth_RS_DS_sigma_050.png}}
    \caption{\textbf{Varying the number of iterations in certification $K$.} The left figure shows certification with $\sigma=0.12$ on CIFAR10 and $\sigma=0.5$ on ImageNet.
    }
        \label{fig:iteration}
        \vspace{-0.65cm}
\end{figure}



==> Data-Dependent Randomized Smoothing-camera-ready/figs/pull.tex <==
\begin{figure}
    \centering
    \includegraphics[width =\linewidth]{figures/pull.png}
    % \vspace{-0.35cm}
    \caption{\textbf{From fixed to data dependent smoothing.} Using a fixed $\sigma$ for all inputs to smooth $f_\theta$ may under certify (results in smaller certification radius) inputs far from decision boundary \eg $x_1$, decrease in prediction confidence as for $x_2$ or produce incorrect predictions as for $x_3$. Thus, smoothing should vary per input (right figure) to alleviate the aforementioned issues.}
    % , larger smoothing for inputs far from decision boundary and vice verse.}
    % \bibi{we should change $x_2$ to have $x_3$ on top and $x_2$ in the bottom. In $x_2$ (which will be $x_3$ we need to tilt the decision boundaries to make it obvious that prediction changed. We also should change sigma in title to $\sigma$.}
    % \motasem{Changes are made.}
    \label{fig:pull_fig}
    % \vspace{-0.55cm}
\end{figure}


==> Data-Dependent Randomized Smoothing-camera-ready/figs/qualitative.tex <==
\begin{figure}[t]
         \centerline{
         \includegraphics[width=0.3\linewidth]{  visualizations/Cohen/minsigma0_0.5_clean.png} 
         \includegraphics[width=0.3\linewidth]{  visualizations/Cohen/minsigma0_0.5.png} 
         \includegraphics[width=0.3\linewidth]{  visualizations/Cohen/minsigma0_0.5_sigma_0.368.png}
         }\centerline{
         \includegraphics[width=0.3\linewidth]{  visualizations/SmoothAdv/maxsigma0_0.25_clean.png}
         \includegraphics[width=0.3\linewidth]{  visualizations/SmoothAdv/maxsigma0_0.25.png}
         \includegraphics[width=0.3\linewidth]{  visualizations/SmoothAdv/maxsigma0_0.25_sigma_0.423.png}}
     \caption{\textbf{Qualitative examples of estimated $\sigma^*_x$ on different inputs.} From left to right of first row: clean image, fixed $\sigma=0.5$  and estimated $\sigma^*_x=0.368$ maximizing certification radius. Similarly for second row but with $\sigma=0.25$ and $\sigma^*_x=0.423$. This demonstrates that $\sigma^*$ that maximizes the radius should vary per input $x$.
    %  where a sub optimal global $\sigma$ can hurt certification.
     }
        \label{fig:qualitative}
        % \vspace{-0.65cm}
\end{figure}


==> Data-Dependent Randomized Smoothing-camera-ready/tables/Cohen.tex <==
\begin{table*}[t]
% \small
\centering
\caption{\textbf{Best certified accuracy per radius and ACR}
% We compare the best certified accuracy and ACR 
of $\text{Cohen}$, $\text{Cohen-DS}$ and $\text{Cohen-DS}^2$.}
% per radius on both CIFAR10 and ImageNet.}
% \vspace{-0.25cm}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cc| ccccccccccc |c}
\toprule 
\midrule
    \multirow{2}{*}{\textcolor{red}{CIFAR10}} & \multicolumn{2}{c|}{Radius}  & \multirow{2}{*}{0.0} & \multirow{2}{*}{0.25} & \multirow{2}{*}{0.50} & \multirow{2}{*}{0.75} & \multirow{2}{*}{1.00} & \multirow{2}{*}{1.25} & \multirow{2}{*}{1.50} & \multirow{2}{*}{1.75} & \multirow{2}{*}{2.00}& \multirow{2}{*}{2.25} & \multirow{2}{*}{2.50}& \multirow{2}{*}{\text{ACR}}\\
    & \text{Train} & \text{Certify} &  &&&&&&& &\\
\midrule
\text{Cohen} & \text{FS} & \text{FS} &\textbf{79.9}& 58.3& 40.1& 29.2& 20.2& 13.1& 7.3& 3.3& 0.0& 0.0& 0.0& 0.591 \\
\text{Cohen-DS} & \text{FS} & \text{DS}&77.2& 64.5& 47.8& 38.3& 27.6& 16.5& 8.0& 3.2& 1.2& \textbf{0.7}& \textbf{0.5}& \textbf{0.784}\\
$\text{Cohen-DS}^2$ & \text{DS} & \text{DS}&79.8& \textbf{66.5}& \textbf{50.4}& \textbf{39.2}& \textbf{29.1}& \textbf{18.3}& \textbf{8.8}& \textbf{3.8}& \textbf{1.4}& 0.6& 0.2& 0.764\\
\midrule
\midrule
    \multirow{2}{*}{\textcolor{red}{ImageNet}} & \multicolumn{2}{c|}{Radius}  & \multirow{2}{*}{0.0} & \multirow{2}{*}{0.25} & \multirow{2}{*}{0.50}& \multirow{2}{*}{0.75}  & \multirow{2}{*}{1.00} & \multirow{2}{*}{1.50} & \multirow{2}{*}{2.0} & \multirow{2}{*}{2.5} & \multirow{2}{*}{3.0}& \multirow{2}{*}{3.50}& \multirow{2}{*}{4.0} & \multirow{2}{*}{\text{ACR}}\\
    & \text{Train} & \text{Certify} &  &&&&&&& &\\
\midrule
\text{Cohen} & \text{FS} & \text{FS} &66.6& 58.2& 49.0& 42.4& 37.4& 27.8& 19.4& 14.4& 12.0& 8.6& 0.0& 1.098
\\
\text{Cohen-DS} & \text{FS} & \text{DS}&\textbf{67.8}& 61.4& 53.6& 45.6& \textbf{42.0}& 30.4& 23.4& 18.8& 14.6& 10.2& \textbf{2.0}& 1.257\\
$\text{Cohen-DS}^2$ & \text{DS} & \text{DS}&67.4& \textbf{64.2}& \textbf{58.4}& \textbf{47.4}& 41.8& \textbf{31.8}& \textbf{25.0}& \textbf{21.2}& \textbf{17.2}& \textbf{11.0}& \textbf{2.0}& \textbf{1.319}\\
\midrule
\bottomrule
\end{tabular}
}
\label{tb:Cohen}
% \vspace{-0.25cm}
\end{table*}

==> Data-Dependent Randomized Smoothing-camera-ready/tables/MACER.tex <==

\begin{table*}[t]
\small
\centering
\caption{\textbf{Best certified accuracy per radius and ACR}
of $\text{MACER}$, $\text{MACER-DS}$ and $\text{MACER-DS}^2$  on CIFAR10.}
% \vspace{-0.25cm}
\resizebox{\linewidth}{!}{
\centering
\begin{tabular}{c|cc| ccccccccccc |c}
\toprule 
\midrule
    \multirow{2}{*}{\textcolor{red}{CIFAR10}} & \multicolumn{2}{c|}{Radius}  & \multirow{2}{*}{0.0} & \multirow{2}{*}{0.25} & \multirow{2}{*}{0.50} & \multirow{2}{*}{0.75} & \multirow{2}{*}{1.00} & \multirow{2}{*}{1.25} & \multirow{2}{*}{1.50} & \multirow{2}{*}{1.75} & \multirow{2}{*}{2.00}& \multirow{2}{*}{2.25}& \multirow{2}{*}{2.50} & \multirow{2}{*}{\text{ACR}}\\
    & \text{Train} & \text{Certify} &  &&&&&&& &\\
\midrule
$\text{MACER}$  &\text{FS} &  \text{FS}        & 78.8& 59.3& 43.6& 34.7& 26.6& 19.4& 13.0& 7.50& 0.0& 0.0 & 0.0& 0.702\\
$\text{MACER-DS}$ &\text{FS} &  \text{DS}        &  79.5& 66.7& 52.3& 43.0& 30.8& 19.5& 12.8& 7.55& \textbf{3.97}& \textbf{1.67}& \textbf{0.5}& \textbf{0.841}\\
% $\text{MACER-DS}^2 (n=1)$  & \text{DS} &  \text{DS}        &  79.6& 61.6& 47.0& 38.2& 29.0&\textbf{20.6}& \textbf{14.4}& \textbf{8.73}& \textbf{4.27}& \textbf{1.70} & \textbf{0.7}& 0.828\\
% \midrule 
% \hline
$\text{MACER-DS}^2$ 
&\text{DS} &  \text{DS}        &  \textbf{82.4}& \textbf{68.3}& \textbf{52.7}& \textbf{43.5}& \textbf{31.7}& \textbf{20.6}& \textbf{13.8}& \textbf{7.92}& 3.65& 1.39& 0.4 & 0.807\\
\midrule
\bottomrule
\end{tabular}
}
\label{tb:MACER}
% \vspace{-0.25cm}
\end{table*}


==> Data-Dependent Randomized Smoothing-camera-ready/tables/SmoothAdv.tex <==
\begin{table*}[t]
\small
\centering
\caption{\textbf{Best certified accuracy per radius and ACR}
% We compare the best certified accuracy and ACR 
of $\text{SmoothAdv}$, $\text{SmoothAdv-DS}$ and $\text{SmoothAdv-DS}^2$.
% per radius on both CIFAR10 and ImageNet.
}
\resizebox{\linewidth}{!}{
% \vspace{-0.25cm}
\centering
\begin{tabular}{c|cc| ccccccccccc |c}
\toprule 
\midrule
    \multirow{2}{*}{\textcolor{red}{CIFAR10}} & \multicolumn{2}{c|}{Radius}  & \multirow{2}{*}{0.0} & \multirow{2}{*}{0.25} & \multirow{2}{*}{0.50} & \multirow{2}{*}{0.75} & \multirow{2}{*}{1.00} & \multirow{2}{*}{1.25} & \multirow{2}{*}{1.50} & \multirow{2}{*}{1.75} & \multirow{2}{*}{2.00}& \multirow{2}{*}{2.25} & \multirow{2}{*}{2.50}& \multirow{2}{*}{\text{ACR}}\\
    & \text{Train} & \text{Certify} &  &&&&&&& &\\
\midrule
\hline
$\text{SmoothAdv}$ & \text{FS} & \text{FS}&76.0& 62.4& 46.7& 34.6& 26.5& 19.5& 12.9& 7.5& 0.0& 0.0& 0.0& 0.681\\
$\text{SmoothAdv-DS}$& \text{FS} & \text{DS}&75.7& 66.4& 52.1& 38.8& 30.6& 22.2& 15.0& 8.5& 4.2& 1.8& 0.6& 0.799\\
$\text{SmoothAdv-DS}^2$ & \text{DS} & \text{DS}&\textbf{76.2}& \textbf{66.8}& \textbf{52.8}& \textbf{39.3}& \textbf{30.8}& \textbf{22.6}& \textbf{15.1}& \textbf{8.8}& \textbf{4.3}& \textbf{2.0}& \textbf{0.7}& \textbf{0.812}\\
\midrule
\midrule
    \multirow{2}{*}{\textcolor{red}{ImageNet}} & \multicolumn{2}{c|}{Radius}  & \multirow{2}{*}{0.0} & \multirow{2}{*}{0.25} & \multirow{2}{*}{0.50}& \multirow{2}{*}{0.75}  & \multirow{2}{*}{1.00} & \multirow{2}{*}{1.50} & \multirow{2}{*}{2.0} & \multirow{2}{*}{2.5} & \multirow{2}{*}{3.0}& \multirow{2}{*}{3.50}& \multirow{2}{*}{4.0} & \multirow{2}{*}{\text{ACR}}\\
    & \text{Train} & \text{Certify} &  &&&&&&& &\\
\midrule 
\hline
$\text{SmoothAdv}$ & \text{FS} & \text{FS} & 60.8& 57.8& 54.6& 50.4& 42.2& 35.6& 25.6& 20.4& 18.0& 14.2& 0.0& 1.287\\
$\text{SmoothAdv-DS}$ & \text{FS} & \text{DS}&62.0& 60.4& 57.4& 53.2& 47.0& 39.2& 29.2& 23.8& 19.6& 15.2& \textbf{6.2}& 1.445\\
$\text{SmoothAdv-DS}^2$ & \text{DS} & \text{DS}&\textbf{62.2}& \textbf{60.6}& \textbf{58.8}& \textbf{54.2}& \textbf{48.2}& \textbf{43.0}& \textbf{30.6}& \textbf{25.4}& \textbf{21.6}& \textbf{18.6}& 4.2&\textbf{1.514} \\
\midrule
\bottomrule
\end{tabular}
}
\label{tb:SmoothAdv}
% \vspace{-0.25cm}
\end{table*}

==> Data-Dependent Randomized Smoothing-camera-ready/tables/l1.tex <==
\begin{table}[t!]
  \caption{\textcolor{black}{\textbf{Best certified accuracy per $\ell_1$ radii and ACR} of \textsc{Yang} and \textsc{Yang-DS}.  }}
  \label{tab:l1}
%   \small
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{l|cccccccc}
    \toprule
    \midrule
    \textcolor{red}{$\ell_1^r$(CIFAR10)} & 0.0 & 0.25 & 0.5 & 0.75 & 1.0 & 1.5 & 2.0 & ACR\\
    \midrule
     \textsc{\texttt{Yang}} & 92 & 83 & 75 & 71 & 46 & 0 & 0 & 0.775      \\
     \textsc{\texttt{Yang-DS}}&  92 & \textbf{89} & \textbf{82} & \textbf{76} & \textbf{58} & \textbf{6} & \textbf{2}& \textbf{0.946}      \\
    \midrule
    \midrule
    \textcolor{red}{$\ell_1^r$(ImageNet)} & 0.0 & 0.25 & 0.5 & 0.75 & 1.0 & 1.5 & 2.0 & ACR\\
    \midrule
      \textsc{\texttt{Yang}} & 78 & 73 & 67 & 63 & 0 & 0 & 0 & 0.683    \\
     \textsc{\texttt{Yang-DS}}& \textbf{79} & \textbf{76} & \textbf{70} & \textbf{65} & \textbf{46} & 0 & 0 & \textbf{0.729}     \\
     \midrule
    \bottomrule
  \end{tabular}}
\end{table}




==> Sections/UAI_rebuttal.tex <==
\newpage
\section{Rebuttal}
\subsection{bfhi Score:5 Confidence:4}


\paragraph{Our response.} We thank the reviewer for the detailed feedback. We address the raised concerns from the reviewer in the same order. We are glad that the reviewer found the idea novel and intriguing and that it has a potential high impact within a subfield of AI.

\textbf{A memory-based based classifier means that its performance will depend on the data it previously saw, and it also depends on the order data comes in.} In general, the reviewer is correct about their observation and we have openly discussed this in the paper as stated in the Limitations Section E of the Appendix. However, observe that memory based certification is order dependent only if two differently predicted samples have overlapping certified regions, i.e. when either the middle or right most cases on Figure 2 occur. That is to say, if overlapping certified regions of different predictions does not occur, the memory based approach is order invariant. A natural question that arises is: ``How likely is it to have two certified regions, note that they are often of $\ell_2$ order of 1.0, intersect for two differently predicted samples?" We observe that this is far unlikely to occur, unless the accuracy of the classifier is poor. During memory based certification, we observe that for all experiments conducted on the respective datasets, this scenario does not happen. This implies that all reported certified accuracies in the paper are in fact the same for any arbitrary order of testing samples of the respective datasets.


\textbf{It seems to me it will become harder and harder to certify when more points are in memory. If there are infinite number of data coming in, what is the asymptotic performance of the proposed method? Would certified accuracy drop to 0 asymptotically? And how does the order of data affect its asymptotic performance?} The observation of dense ``infinite" data for testing is partially true. While indeed the more samples tested the more likely for an intersection of certified regions to happen, however, it is not necessarily the case that the intersections of certified regions of differently predicted samples will increase. To that end, this does not mean that all new samples will later be necessarily certified with consecutively smaller regions, as observed on the respective datasets, since intersected regions of differently classified samples are rare. However, this naturally suggests an interesting direction. A stronger adversary is one with a full access to the history of all previously tested samples in memory. Such an attacker can then present few malicious samples for testing that will go in memory such that for future samples this can cause the data dependent classifier to intersect with higher chances with previously differently predicted samples causing certified accuracy to asymptotically drop for future samples. While this adversary could exist in principal, it is also not practically of full relevance. This is since in practice classifiers at deployment get updated in which new classifiers with fresh new memory are to be certified. In general, this is an interesting future research direction, but currently, a definition of such a class of adversaries falls beyond the scope of our paper.

% Moreover, even in classical certification, attaining a certain certified accuracy performance on a dataset reflects the performance of such adversary

\textbf{Following the methodology in this paper, conceptually, we can also discard all the remembered certifications in memory, and start fresh with a new classifier each time. Essentially this means we are using one fresh classifier for each example. Is it possible to do so and what is the implication?} If one resets the memory and provide certification for every sample independently along with a certified radius, the best one can deduce from such a classifier is that if $x+\delta$ is presented to the classifier, to attain a sound certification, the same $\sigma$ used for $x$ should also be used for $x+\delta$. If such a condition can not be practically deployed, we only end up with a theoretical classifier (since we do not have a procedure to implement such a classifier with a constant $\sigma$ locally) that is with a sound certification. Thus, the memory here is to allow for a practical implementation of this classifier with a sound practical certification. Thus if the memory is reset consecutively when testing every one of the new $n$ samples, we are at either (1) providing a sound certification of $n$ tested samples for a theoretical classifier or (2) providing $n$ sound certifications for $n$ different smooth classifiers (each with a different $\sigma$). This is where the use of memory bridges this gap into providing a single practical classifier with a sound certification.



% This is since the randomized smoothing certification suggests that given $x$ if for all samples $x+\delta$ in the certified region of $x$ denoted as $\mathcal{R}(x)$ is predicted with a constant $\sigma$ prediction does not change.


\textbf{Is it possible to achieve soundness without memory?} Currently, we do not have any particular obvious approach to drop the dependence on previous samples for certification. This could be a potential future direction that we currently do not yet know how to approach.





% Note that as mentioned in Section 3.5, we found that this is the case in all of our experimental results where no instances with differently predicted labels share any overlap in their certified regions making our memory-enhanced classifier order invariant. 


\subsection{S8Ji Score:7 Confidence:3}
We thank the reviewer for the valuable and detailed comments. We are glad that our work was well-received by the reviewer.

\textbf{Regarding the dependent of the memory algorithm on the order.} Indeed, the reviewer comment is on spot in their observation. The memory algorithm is order dependent. We have openly discussed this in the paper as stated in the Limitations Section E of the Appendix. However, this drawback had no impact in all of our experimental results. As discussed in our response to Rerviewer bfhi, memory based certification is order dependent only if two differently predicted samples have overlapping certified regions, i.e. when either the middle or right most cases in Figure 2 occur. That is to say, if overlapping certified regions of different predictions does not occur, the memory based approach is order invariant. We observe that this it is is far to have intersection of two different certified regions of differently predicted samples. In all our experiments, we observe that this scenario does not happen (middle and right most settings of Figure 2). This implies that all reported certified accuracies in the paper are in fact the same for any arbitrary order of testing samples of the respective datasets.

\textbf{Regarding the constrained covariance matrix.} We agree with reviewer S8Ji. Anisotropic covariance matrices could increase the certified volume. However and for a fair comparison with earlier approaches such as SmoothADV and MACER, we devoted our analysis in this work for isotropic covariance matrices leaving the anisotropic counterparts for a future work. Moreover, considering full covariance matrices requires (1) deriving the resultant certificate (e.g. ellipsoid as opposed to $\ell_2$ balls) (2) defining a new approach towards comparing two anisotropic certified regions through volumes or other metrics.

\textbf{Regarding learning or predicting the variance.} This is an excellent idea that would alleviate the optimization cost of obtaining the optimal smoothing parameters. However, we argue that learning/predicting the smoothing parameters is a very challenging problem that could potentially reduce the improvement of using data dependent smoothing. We have had initial experiments of learning a separate network to predict $\sigma$ for the sole purpose of speeding up certification as this involves a forward pass through a network as opposed to solving the optimization problem. However, we do not find any particular gains, in fact this approach down performs the classical baselines as Cohen et al. We leave the investigation for this line of work for a future direction.


\subsection{MTkP Score:7 Confidence:3}
We thank the reviewer for the valuable and detailed comments. We are glad that our work was well-received by the reviewer.

\textbf{Regarding the runtime comparison}: We thank the reviewer for pointing out this fair comparison. We have included a detailed comparison of the running time in Appendix H. We will include this paragraph in the main paper in the final version.


\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{UAI22/rebuttal_figures/cohen_comparison_0.25.pdf}
    \caption{Rebuttal Experiment}
    \label{fig:rebuttal_experiment}
\end{figure}


\textbf{Regarding the minor issues.} We thank the reviewer for this insightful experiments. As suggested, we conducted this experiment for Cohen baseline at $\sigma=0.25$. We plot the histogram of the obtained $\sigma_x^*$ for CIFAR10 in orange. We also plot a histogram of the $\sigma_x^*$ at which the certified radius is improved in green. We report the results in Figure~\ref{fig:rebuttal_experiment}.
We found that the certified robustness improvements happen at the full spectrum of $\sigma_x^*$ showing the efficacy of our proposed data-dependent smoothing. We will include a more detailed version of this experiment in the final version.



\textbf{Regarding the proposed adjustment for the middle scenario in Fig 2.} The reviewer is correct about their observation and suggestion. We opted to the solution with the least computational overhead which is adjusting the radius of the new data as opposed to adjusting the radius of every intersected sample in memory. We would like to bring to the attention of the reviewer that in practice, given that the certified regions around every point is generally small, scenarios 2 and 3 in Figure 2 never happened on the correspondingly tested datasets, i.e. there are no differently predicted samples with intersected certified regions.

% However, better alternatives could exist that could potentially result in a better overall certified radius.
% There might exist many solutions for this case such as the one pointed out by the reviewer.


\textbf{Regarding $\hat x$ and $x'$}. Yes, this is indeed a typo where the optimization is over the adversary $x'$. We will correct this in a potential future version.

% We refer to $\hat x$ as the adversarial attack. $x'$ is the optimization variable in the objective:
% \[\max_{x'} -\log \mathbb {E}_{\epsilon \sim \mathcal N (0,\sigma^2I)} \left[f^y_{\theta}(x' + \epsilon)\right], \qquad \text{where}\quad \|x'-x\| \leq \zeta
% \]
% We will make this clearer in the final version.







\subsection{7p67 Score:7 Confidence:2}
We thank the reviewer for the valuable and detailed comments. We are glad that our work was very well-received with generally positive feedback by the reviewer.

\textbf{Regarding the presentation details.} We thank the reviewer for spotting some typos and fir suggesting several few ways to improve presentation. We will surely address those in any potential camera ready version.

% We have used the command eqref to refer to previous equations so that the reader could click on it to jump directly to the equation. We will fix this as per the suggestion and add paranthesis for better clarification.

% (2) We thank the reviewer for spotting this clerical error which will be fixed in the final version.

\textbf{Regarding predicting $\sigma^*$ for any $x$.} We thank the reviewer for sharing this interesting idea. We thought about learning $\sigma_x^*$ through a network that is jointly trained with the classifier. However, and due to the hardness of the problem, we were not able to attain robustness improvements from that approach over the Cohen et al baseline. The loss function used is similar to Equation 2, but the optimization is over parameters $\phi$ of an encoder network where $\epsilon$ is sampled from the encoder network. This is in similar spirit to variational autoencoders (VAEs). The reason for why this approach did not work could be attributed to several factors such as the poor performance of the classifier at early epochs, the complexity of the optimization, etc. Nevertheless, we believe that such approaches, if succeeded, would have several advantages such as alleviating the optimization cost.

==> figs/iteration_ablation.tex <==
\begin{figure}[t]\vspace{-0.2cm}
\centerline{
     \includegraphics[width=0.24\textwidth]{figures/iterations/CIFAR10_Adv_smooth_DS_DS_sigma_012.png}\hfill
    \includegraphics[width=0.24\textwidth]{figures/iterations/ImageNet_Adv_smooth_RS_DS_sigma_050.png}}
    \caption{\textbf{Varying the number of iterations in certification $K$.} The left figure shows certification with $\sigma=0.12$ on CIFAR10 and $\sigma=0.5$ on ImageNet.
    }
        \label{fig:iteration}
        \vspace{-0.65cm}
\end{figure}


